ADMM-MCBF-LCA: A Layered Control Architecture for Safe Real-Time Navigation

We consider the problem of safe real-time navigation of a robot in a dynamic environment with moving obstacles of arbitrary smooth geometries and input saturation constraints. We assume that the robot detects and models nearby obstacle boundaries with a short-range sensor and that this detection is error-free. This problem presents three main challenges: i) input constraints, ii) safety, and iii) real-time computation. To tackle all three challenges, we present a layered control architecture (LCA) consisting of an offline path library generation layer, and an online path selection and safety layer. To overcome the limitations of reactive methods, our offline path library consists of feasible controllers, feedback gains, and reference trajectories. To handle computational burden and safety, we solve online path selection and generate safe inputs that run at 100 Hz. Through simulations on Gazebo and Fetch hardware in an indoor environment, we evaluate our approach against baselines that are layered, end-to-end, or reactive. Our experiments demonstrate that among all algorithms, only our proposed LCA is able to complete tasks such as reaching a goal, safely. When comparing metrics such as safety, input error, and success rate, we show that our approach generates safe and feasible inputs throughout the robot execution.

==> commands.tex <==
\newcommand{\yifan}[1]{{\color{red}{Yifan: #1}}}
\newcommand{\anusha}[1]{{\color{blue}{Anusha: #1}}}

\newcommand{\rev}[1]{\textcolor{red}{#1}}

 
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{coro}[theorem]{Corollary} 
%\newtheorem{remark}{Remark}

%\numberwithin{equation}{section}

%\newtoggle{draft}
%\toggletrue{draft}
%\togglefalse{draft}

\newcommand{\todo}[1]{
\iftoggle{draft}{
\vspace{5 mm}\par \noindent \marginpar{\textsc{ToDo}}
\framebox{\begin{minipage}[c]{0.95 \columnwidth} \tt #1
\end{minipage}}\vspace{5 mm}\par}{}}

\newcommand{\propchange}[1]{
\iftoggle{draft}{
	{\leavevmode\color{blue}{#1}}}{\leavevmode{#1}}}

\newcommand{\propdelete}[2]{
\iftoggle{draft}{
\textcolor{blue}{\sout{#1} {#2}}}{#2}}


\newcommand{\minimize}{\mbox{minimize}}
\newcommand{\maximize}{\mbox{maximize}}
\newcommand{\st}{\mbox{subject to}}
\newcommand{\statespace}[4]{\left[ \begin{array}{c|c} #1 & #2 \\ \hline #3 & #4 \end{array} \right]}
\newcommand{\tf}[1]{\boldsymbol{#1}}
\newcommand{\Ah}{\widehat{A}}
\newcommand{\Ahat}{\Ah}
\newcommand{\Bhat}{\Bh}
\newcommand{\Bh}{\widehat{B}}
\newcommand{\Kh}{\widehat{K}}
\newcommand{\Jh}{\widehat{J}}
\newcommand{\Phixh}{\hat{\tf \Phi}_x}
\newcommand{\Phiuh}{\hat{\tf \Phi}_u}
\newcommand{\Phix}{\tf\Phi_x}
\newcommand{\Phiu}{\tf\Phi_u}
\newcommand{\Phih}{\hat{\tf \Phi}}
\newcommand{\Dh}{\hat{\tf{\Delta}}}
\newcommand{\DA}{\D_{\A}}
\newcommand{\DB}{\D_{\B}}
\newcommand{\trueA}{A}
\newcommand{\trueB}{B}
\newcommand{\trueK}{K_\star}
\newcommand{\A}{\tf A}
\newcommand{\K}{\tf K}
\newcommand{\Q}{\tf Q}
\newcommand{\xhat}{\tf{\hat x}}
\newcommand{\what}{\hat{\tf w}}
\newcommand{\eps}{\varepsilon}
\newcommand{\R}{\mathbb{R}}
\newcommand{\M}{\mathbb{S}}

\DeclareMathOperator*{\argmin}{arg\!\min}
\DeclareMathOperator*{\argmax}{arg\!\max}
\DeclareMathOperator*{\sgn}{sgn}
\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\Tr}{\mathbf{Tr}}
\DeclareMathOperator*{\image}{Im}
\DeclareMathOperator*{\nullspace}{Kern}
\DeclareMathOperator*{\rowspace}{RS}
\DeclareMathOperator*{\colspace}{CS}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\vol}{vol}
\DeclareMathOperator*{\Span}{span}
\DeclareMathOperator*{\polylog}{polylog}
\DeclareMathOperator*{\Band}{Band}
\newcommand{\grad}{\mathrm{grad}}
\newcommand{\bias}{\mathrm{Bias}}
\newcommand{\var}{\mathrm{Var}}


\newcommand{\ltwonorm}[1]{\| #1 \|_2}
\newcommand{\hinfnorm}[1]{\| #1 \|_{\hinf}}
\newcommand{\bighinfnorm}[1]{\left \| #1 \right\|_{\hinf}}
\newcommand{\bightwonorm}[1]{\left \| #1 \right\|_{\htwo}}
\newcommand{\iid}{\stackrel{\mathclap{\text{\scriptsize{ \tiny i.i.d.}}}}{\sim}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\infty}}
\newcommand{\linfnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\LTV}{\mathcal{L}_{\mathrm{TV}}}
\newcommand{\LTI}{\mathcal{L}_{\mathrm{TI}}}
\newcommand{\linffnorm}[1]{\left\|#1\right\|_{\ell_\infty\to\ell_\infty}}
\newcommand{\Sp}{\tf S_+}
\newcommand{\Sm}{\tf S_-}
\newcommand{\RHinf}{\mathcal{RH}_\infty}
\newcommand{\RLinf}{\mathcal{RL}_\infty}

\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\cbf}{h}
\newcommand{\cbfe}{h_{exp}}
\newcommand{\statedim}{n}
\newcommand{\inputdim}{m}
\newcommand{\xx}{x}
\newcommand{\yy}{y}
\newcommand{\uu}{u}
\newcommand{\g}{g}
\newcommand{\q}{q}
\newcommand{\f}{f}
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\newcommand{\Ss}{\ensuremath{\mathcal{S}}}
\newcommand{\Ds}{\ensuremath{\mathcal{DS}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\bD}{\ensuremath{{\bar{\mathcal{D}}}}}
\newcommand{\C}{\ensuremath{\mathcal{C}}}
\newcommand{\Ce}{\ensuremath{\mathcal{C}_{exp}}}
\newcommand{\N}{\ensuremath{\mathcal{N}}}
\newcommand{\Pp}{\ensuremath{\mathcal{P}}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\U}{\ensuremath{\mathcal{U}}}
\newcommand{\B}{\ensuremath{\mathcal{B}}}
\newcommand{\Lc}{L_h}
\newcommand{\Ln}{L_\nabla}
\newcommand{\Lq}{L_q}
\DeclareMathOperator*{\bd}{bd}
\DeclareMathOperator*{\cl}{cl}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\inte}{int}
\newcommand{\norm}[1]{\| #1 \|}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Lip}{\mathrm{Lip}}

\newcommand{\calF}{\mathcal{F}}

\newcommand{\Xsafe}{X_{\mathrm{safe}}}
\newcommand{\bXsafe}{\bar{X}_{\mathrm{safe}}}
\newcommand{\Xunsafe}{X_{\mathrm{unsafe}}}
\newcommand{\Xboundary}{X_{\mathrm{bound}}}
\newcommand{\gammasafe}{\gamma_{\mathrm{safe}}}
\newcommand{\gammaunsafe}{\gamma_{\mathrm{unsafe}}}
\newcommand{\gammaboundary}{\gamma_{\mathrm{bound}}}
\newcommand{\XN}{X_{\mathcal{N}}}
\newcommand{\XS}{X_{\mathcal{S}}}
\newcommand{\Zdynamics}{Z_{\mathrm{dyn}}}
\newcommand{\gammadynamics}{\gamma_{\mathrm{dyn}}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calH}{\mathcal{H}}

\newcommand{\ip}[2]{\langle #1, #2 \rangle}
\newcommand{\T}{\mathsf{T}}
\newcommand{\abs}[1]{| #1 |}
\def\lc{\left\lceil}   
\def\rc{\right\rceil}
\def\lf{\left\lfloor}   
\def\rf{\right\rfloor}

\newcommand{\vertexset}{\mathcal{V}}
\newcommand{\edgeset}{\mathcal{E}}
\newcommand{\dist}{\mathbf{dist}}
\newcommand{\infoset}{\mathcal{J}}
\newcommand{\totalinfoset}{\mathcal{I}}
\newcommand{\incoming}{\mathbf{in}}
\newcommand{\vectorize}[1]{\textrm{vec}(#1)}
\newcommand{\kron}{\ensuremath{\otimes}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}
\def\gN{{\mathcal{N}}}
\def\ermS{{\textnormal{S}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

%\newcommand{\comment}[1]{}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\ch}[1]{\textcolor{black}{#1}}
\newtheorem{example}{Example}

\def\ctrl{{\mathcal{K}}}

%BEGIN SHORTHANDS
% -- Shorthands --
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
% \newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
% \newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
% \newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}

==> tex/0-abstract.tex <==
\begin{abstract}
    % Discuss how ADMM applied to OCP gives you a nominal long-horizon controller that is guaranteed to be input feasible. Further, in the shorter horizon, ADMM run for a fixed number of iterations
   We consider the problem of safe real-time navigation of a robot in a dynamic environment with moving obstacles of arbitrary smooth geometries and input saturation constraints. We assume that the robot detects and models nearby obstacle boundaries with a short-range sensor and that this detection is error-free. This problem presents three main challenges: i) input constraints, ii) safety, and iii) real-time computation. To tackle all three challenges, we present a layered control architecture (LCA) consisting of an offline path library generation layer, and an online path selection and safety layer. To overcome the limitations of reactive methods, our offline path library consists of feasible controllers, feedback gains, and reference trajectories. To handle computational burden and safety, we solve online path selection and generate safe inputs that run at $100$ Hz. Through simulations on Gazebo and Fetch hardware in an indoor environment, we evaluate our approach against baselines that are layered, end-to-end, or reactive. Our experiments demonstrate that among all algorithms, only our proposed LCA is able to complete tasks such as reaching a goal, safely. When comparing metrics such as safety, input error, and success rate, we show that our approach generates safe and feasible inputs throughout the robot execution.
   % The offline layer consists of nominal controller library generation, while the online layer handles real-time execution through path selection and guaranteed reactive obstacle avoidance. 
   % Using our proposed framework, we empirically show that careful and efficient algorithmic design of feasible nominal feedback controllers significantly improves robustness to model uncertainties for differential drive robots. 
   % We verify this by comparing against purely reactive methods for obstacle avoidance that use infeasible nominal inputs. 
   % We also argue the need for long-horizon \emph{multi-path} nominal controllers compared to real-time model predictive control which results in suboptimal performance due to uncertainties and computational constraints. Our simulation experiments in an indoor environment with unknown obstacles indicate that only our proposed solution guarantees safety while resulting in convergence to the goal. We also demonstrate that our proposed layered solution outperforms baselines in terms of safety, and input tracking error.
   
   % Our approach provides a real-time algorithm that guarantees safe This problem presents two many challenges such as real-time computation, task completion and safety. Prior work from optimization-based control design reactive policies that guarantee safety but are limited by nominal inputs., however, A widely used solution modifies nominal controllers by solving a quadratic program (QP) with a control barrier function (CBF) constraint called CBF-QP. However, the performance of CBF-QPs are governed by the design of nominal controllers for ensuring task completion. By using  Using model predictive controllers To overcome the limitation of CBF-QPs, prior work designs a model predictive controller (MPC) with a discrete-time CBF constraint in the OCP. However, MPC-CBF methods result in suboptimal performance for very short horizons selected due to computational constraints. Therefore, to achieve real-time performance while ensuring task completion, we propose a layered solution consisting of a library of nominal controllers in the top layer, a trajectory selector in the middle layer, and a reactive safety filter in the lowest layer. Based on user design choices of inter-trajectory intervals and waypoints per trajectory, we generate each nominal controller consisting of a feedforward term and a feedback gain matrix offline by solving OCP via alternating direction method of multipliers (ADMM). During execution, we modify the nominal feedback control using a CBF safety filter to guarantee obstacle avoidance. We measure the deviation in current state and the library of nominal states to select the path that the controller should follow using nearest neighbor search. 
    % The resulting controller consists of a feedforward term that guides the system to the target, and a feedback gain matrix to locally stabilize the system around the nominal trajectory. 
    % We perform trajectory selection online using a nearest neighbor search over predicted next states, while obstacle avoidance is handled via control barrier functions, meeting real-time computational requirements. 
    
    
    % We provide empirical evaluations using numerical simulations for a Dubins car dynamics model in complex obstacle environments, comparing our layered solution against MPC-CBF and two ablated baselines, one reactive and the other not planning over long horizons. Our results demonstrate that ... Additionally, we evaluate our proposed layered solution on a Fetch robot, showing that our method outperforms both baselines in terms of task completion, safety, comfort, and input tracking error.
    
    % We consider the problem of real-time navigation in an unknown dynamic environment for a robot equipped with a range sensor such as a LiDAR to detect nearby obstacles. This problem poses two key challenges: i) real-time computation, and ii) safe obstacle avoidance. A widely used solution to tackle these challenges involves the use of reactive methods such as a safety filter using control barrier functions (CBFs). However, due to the greedy nature of reactive policies, such approaches fail to complete tasks and get stuck in local minima. Therefore, prior work incorporate future states through the use of model predictive control (MPC) by coupling control objectives and saturation constraints with a discrete-time CBF constraint in an optimal control problem (OCP) to guarantee safety. However, the choice of MPC horizon depends on real-time computational constraints resulting in suboptimal performance for very short horizons. To achieve real-time performance while ensuring task completion, we propose a layered solution that consists of a library of nominal controllers in the top layer, a trajectory selector in the middle layer, and a reactive safety filter in the lowest layer. Each nominal controller is computed offline and consists of a feedfoward term that brings the system to the target and a feedback gain matrix to stabilize the system locally around the nominal trajectory. Trajectory selection using a nearest neighbor search over predicted next states and obstacle avoidance via control barrier functions are carried out online satisfying real-time computational guarantees. We show empirical evaluations on numerical simulations for a Dubins car dynamics model in complex obstacle environments and compare our layered solution against MPC-CBF and two ablative baselines that are either reactive or do not plan over long horizons. Our results show that ... Further, we evaluate our proposed layered solution on a Fetch --- and find that our method outperforms both baselines in terms of task completion, safety, comfort, and input tracking error. 

    % we solve a quadratic program  obtained  Each of the nominal controllers is composed of a feedforward term that brings the system to the target and a feedback gain matrix to stabilize the system locally around the nominal trajectory. In real-time,
    % We present a layered solution to robot navigation with real-time performance and safety guarantees. Leveraging ADMM as an operator splitting method for solving a nonlinear optimal control problem (OCP) for waypoint tracking, we obtain a nominal controller that satisfies waypoint tracking and input constraints. Further, the nominal controller has two degrees of freedom (2DOF) consisting of a feedforward term and a feedback term which is not imposed apriori. By uniformly sampling intermediate waypoints in a parallel fashion, we generate several input-feasible nominal controllers with each path associated with the generated waypoints connecting a given initial location to a goal. In practice, robots have other sources of uncertainties or require a reactive safety layer to avoid obstacles. To incorporate a layer of reactive adaptive control for real-time safety guarantees, we fine-tune on the nominal controller using a CBF-based filter for static and dynamic obstacle avoidance. We validate our approach in several numerical simulations for cartpole, unicycle, and bicycle dynamics. Finally, we show experiments on the Fetch robotic platform comparing against ablative baselines that do not consider one or many aspects of our layered solution to show its benefit.
    % We present a novel approach to real-time obstacle avoidance using a layered control architecture for underactuated robots. Applying alternating direction method of multipliers to a nonlinear optimal control problem with input contraints, we obtain an unconstrained dynamics layer and a separable across time steps feasibility problem with input constraints to obtain a long-horizon nominal controller that strictly satisfies input feasibility. Further, The aim of this paper is to present experimental results validating our theory of layered control architectures applied to robotic systems. We present a decomposition of a nonlinear optimal control problem through the introduction of redundant reference variables to obtain a nominal tracking controller which is further modified using a control barrier function to ensure safety from collisions with static and dynamic obstacles. We show how our approach can be used to make comparisons between different approximate dynamics models used for designing the nominal controller and verify our performance on extensive simulations and on a real robot setting.
\end{abstract}

==> tex/1-Intro.tex <==
\section{Introduction}
% Recent developments in autonomous systems have brought increasing research efforts into the field of robot obstacle avoidance and safe control system design. Autonomous robots colliding with environmental obstacles or their co-workers would not only reduce work efficiency but also injure users in safety-critical tasks ranging from autonomous driving to household human-robot cooperation \cite{ROB-052}.
Historically, motion planning algorithms~\cite{canny1988complexity} decouple the planning problem from feedback control design. The challenge today is to integrate these approaches to ensure safe robot behavior. To this end, layered control architectures (LCAs) offer a design methodology for robot navigation using hierarchical layers balancing constraint complexity and trajectory horizons: see the recent survey~\cite{matni2024towards} which highlights the success of LCAs across robotics and other application areas.  Many works~\cite{rosolia2020multi, grandia2021multi, rosolia2022unified, matni2024towards} employ LCAs where higher layers solve model predictive control (MPC) over long horizons at low frequencies, while lower layers handle trajectory tracking at higher frequencies. However, integrating these layers is challenging due to mismatched time scales, real-time computational requirements, and task completion objectives. Real-time solutions~\cite{stolle2006policies, majumdar2017funnel} often rely on offline libraries of 
% infeasible 
reference trajectories or reachable sets, combined with online planning, but these components assume partial or complete knowledge of the environment and can be difficult to coordinate effectively. 
% In this paper, we propose to generate a path library without assuming access to a map or any knowledge of obstacles. 
In contrast, we assume that obstacles within a local radius are visible to the robot, and aim to ensure safety through reactive control.
% In contrast, we do not assume access to a map or obstacles, but instead assume that the exploration region for the robot is known and aim to guarantee safety.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.597\linewidth}
         \includegraphics[width=\textwidth]{img/fetch_experiment_annotated_gray_trim.png}
    \caption{Safe Real-Time Navigation\label{fig:video}}
\end{subfigure}\hspace{2pt}\begin{subfigure}{0.3899\linewidth}
         \includegraphics[trim={11cm 2cm 17cm 10cm},clip,width=\linewidth]{img/main-hardware-result.png}
     \caption{RVIZ visualization \label{fig:rviz}}
    \end{subfigure}
    \caption{We show a Fetch robot successfully reaching a goal in a dynamic environment running our proposed algorithm to avoid a human walking around and other static obstacles. Blue and green shades in \autoref{fig:rviz} are obstacles, while the green trajectories are ADMM-generated feasible paths. }   
    \vspace{-20pt}
    \label{fig:experiment}
\end{figure}
\vspace{-1.2em}

% Safety-critical robot navigation~\cite{hsu2023safety} in unknown indoor environments faces challenges such as cluttered, dynamic obstacles, nonlinear dynamics, and real-time constraints. 
Although reactive control strategies for safety-critical robot navigation~\cite{hsu2023safety}, such as artificial potential fields~\cite{apf1989real}, navigation functions~\cite{loizou2003closed, loizou2007mixed}, dynamical system (DS) based modulation~\cite{LukesDS,DSTEXTBOOK} and control barrier functions (CBFs)~\cite{ames2019control,notomista2021safety,singletary2021comparative}, are computationally effective; they are limited by their greedy policies for long-horizon planning for control-affine input-constrained systems.
% are often used for dynamic obstacle avoidance due to their computational efficiency. 
Such policies struggle to escape local minima (saddle points) in cluttered non-convex environments that are not ball \cite{notomista2021safety} or star worlds \cite{starworlds} resulting in sub-optimal trajectories and failed mission objectives. 
% This leads to suboptimal trajectories and failed task completion in realistic dynamic environments. 
Further, designing reactive control strategies for nonholonomic vehicles, such as differential drive robots, adds the challenge of contradicting input and safety constraints alongside the use of simplified dynamics models~\cite{planning}. Reactive methods largely rely on a nominal global trajectory encoding task objectives for mission completion. %Task completion for reactive methods largely is governed by the quality of the nominal global trajectory. 
Unlike planning methods that design reference trajectories, we generate path libraries consisting of nominal controllers, feedback gain matrices and reference trajectories. This allows us to relax input constraints at the reactive layer, as we will show, drastically reducing solver infeasibility that plague reactive controllers. 
% is challenging as additional local minima and infeasibilities arise due to i) contradicting input and safety constraints as well as, ii) mismatch between simplified models \cite{planning} and the real-world systems. Finally, the task completion and feasible trajectory generation of all reactive methods also depends on the quality of the nominal global trajectory being tracked. Unlike planning methods that design reference trajectories, we generate path libraries consisting of nominal controllers, feedback gain matrices and reference trajectories. This allows us to relax the enforcement of input constraints at the online execution layer which, as we will show, drastically reduces the infeasibility issues that plague reactive controllers. 

% which we refer to as the nominal controller in this work.

% We also know that CBFs~\cite{singletary2021comparative} inherit similar local minima as their predecessors such as artificial potential fields and navigation functions. We provide comparisons only with CBF or its variants in this paper due to their ease of use in practice for any given obstacle boundary. For nonholonomic vehicles, such as differential drive robots, cannot always be computed in closed form. 
% Even when approximated, these reactive methods can produce infeasible trajectories, leading to stability issues during execution. 

Therefore, in this paper, we offer an LCA that generates an offline library of feasible paths for control-affine input-constrained systems while allowing for smooth transitions between paths with an online path selector that tracks the closest global trajectory with a reactive control strategy ensuring safety in real-time. While one could use any of the aforementioned reactive control strategies, in our proposed LCA framework, we choose the recently introduced on-manifold Modulated CBF method (MCBF)~\cite{xue2024nominima}. The MCBF method applies the notion of on-manifold navigation, initially formulated for DS modulation~\cite{onManifoldMod}, to the CBF safety filter framework eliminating local minima for any arbitrarily shaped obstacle. %The success of this method is attributed to escape velocities on tangent hyperplanes along the obstacle boundaries when saddle points arise.} 
%This method eliminates local minima for any arbitrarily shaped obstacle by generating escape velocities on the tangent hyperplanes of the obstacle boundaries when geometric saddle points arise.

% To the best of our knowledge, on-manifold CBF method (MCBF) ~\cite{xue2024nominima} is the only method that eliminates all saddle-points from CBFs while being applicable to control affine systems. Hence, we use MCBF-QP as a safety filter in our work. However, one can also easily plug in another existing approach with the same properties in our layered framework. 

% Motion planning algorithms~\cite{canny1988complexity} for robot navigation evolved independently of advances in feedback control design. With the availability of sophisticated hardware to solve complex problems, our biggest challenge in robotics today is composing planning algorithms and 
% feedback controllers to ensure safe robot behaviors. To achieve this, experts design a layered control architecture (LCA) in which hierarchical layers tradeoff between constraint complexity and trajectory horizons. A recent survey~\cite{matni2024towards} of LCAs describe the mathematical principles governing their burgeoning success for robot applications through optimization relaxations. Several other works~\cite{rosolia2020multi, grandia2021multi, rosolia2022unified, matni2024towards} use a LCA wherein higher decision making layers solve model predictive control (MPC) at low frequencies over longer horizons while feedback tracking controllers track the generated trajectories via MPC at higher frequencies guaranteeing safety. Alternatively, to achieve real-time performance, layered solutions such as~\cite{stolle2006policies, majumdar2017funnel} generate an offline library of nominal trajectories or reachable sets for a given map of the environment and run a real-time planning algorithm online to select from the offline library of policies. 

Our contributions are as follows.
\begin{enumerate}
    \item To achieve real-time performance while ensuring task completion (e.g., reaching a goal), we propose a layered solution that consists of offline path generation and an online safety filter, as shown in Figure~\ref{fig:intro-block-diag}.
    \item Using the generated library of feasible controllers, feedback gain matrices, and reference trajectories satisfying state constraints, we construct a nominal feedback law that is easy to track for reactive controllers while also ensuring smooth transitions between paths.
    % for each of which we use an efficient algorithm that separates feasibility constraints from dynamics. Further, the separation enables us to compute time-varying feedback gain matrices associated with the offline library of nominal controllers in closed-form. 
    \item With online path selection and a MCBF safety filter that eliminates local minima, we ensure safety in cluttered environments with arbitrarily shaped static and dynamic obstacles. Our online execution layer runs at $100$ Hz.
    \item We provide an open-source implementation of our approach and baselines~\footnote{\url{https://github.com/yifanxueseas/admm_mcbf_lca}}.
    % and tools to specify hyperparameters to ensure the generation of compliant and computationally efficient LCAs.
\end{enumerate}

% We organize the rest of the paper as follows. 
In Section~\ref{sec:related-work}, we discuss prior work from related topics to contextualize our contributions, and introduce the problem in Section~\ref{sec:prob-form}.
% , we introduce our problem statement and define the notion of safety that we use throughout the rest of the paper. 
In Section~\ref{sec:admm-cbf-lca}, we propose our layered framework as shown in Figure~\ref{fig:intro-block-diag} consisting of an offline library generation layer and an online execution layer. In Section~\ref{sec:experiments}, we show comparisons of our method against baselines, highlighting the benefits of layering and long-horizon multi-path offline libraries. We end with concluding remarks in Section~\ref{sec:conclusion}.

% \lipsum[1-2]
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/ICRA-25-figures-block-diagram-final-final-2.pdf}
    \caption{We present a schematic of our approach showing the offline path library generation on the top in blue and online execution in green. We generate a total of $N$ nominal controllers by using a fixed set of waypoints to sufficiently cover the initial known safe set. When commanding the robot, we use nearest neighbor search over predicted next states to choose a path where ties are broken by choosing the one closer to the center. We construct our nominal feedback input and apply a safety filter using a on-Manifold control barrier function. Finally, this is applied to the robot in real-time. 
    % Using the deviation predicted state and measured state, we determine whether the next nominal input or the same one to account for motor delays and uncertainties. %\textbf{NF: Highlight frequencies of these blocks}
    }
    \label{fig:intro-block-diag}
    \vspace{-10pt}
\end{figure*}
% \lipsum[3-10]

\vspace{-.25em}

% Safety-critical robot navigation~\cite{hsu2023safety} in unknown indoor environments presents a challenging control problem due to several factors such as cluttered and dynamic environments, kinematic and nonlinear dynamic constraints, safety, actuator saturation, and real-time computational constraints. Moreover, navigating in unknown dynamic environments in the presence of moving obstacles with a short range obstacle detection sensor begs the need for reactive control strategies. While reactive methods such as the use of control barrier functions (CBFs)~\cite{} as a safety filter for guaranteeing obstacle avoidance are computationally efficient, they result in a greedy policy that do not take into account future predictions. \yifan{Add citations and describe the drawbacks of reactive methods such as local minima etc.} In practice, the performance of CBF-QP controllers are limited by the feasibility of their nominal controllers. For nonholonomic vehicles such as the differential drive, nominal controllers cannot be computed in closed-form, even when robot actuation limits are ignored. Even in cases when nominal controllers can be approximated mathematically using a greedy policy, trajectories resulting from such controllers are not feasible and cause stability issues when tracked by the robot. 

% To design controllers that account for future states, model predictive control (MPC) is widely used in the robotics literature~\cite{borrelli2017predictive, ostafew2016robust} \anusha{add more citations} where at each time step a constrained optimal control problem (OCP) is solved over a fixed horizon, and the first input is applied. By choosing an appropriate terminal cost and terminal constraint, MPC results in locally optimal controllers for nonlinear systems and guarantee feasibility and stability of the closed-loop system~\cite{chen2000model}. However, one of the major challenges for implementing MPC is handling the computational burden of solving nonlinear optimization at each time step. To improve computational efficiency, a rich body of work~\cite{wang2009fast, east2018admm, rey2020admm, gracia2024efficient, krupa2024sparse} exploits the structure from applying the alternating direction method of multipliers (ADMM) algorithm to solving constrained OCPs in MPC. However, most of these approaches are limited to linear settings and none of them prescribe a method to handle time-varying safe sets when new obstacles are detected in the environment during robot navigation. To address safety, prior work called MPC-CBF~\cite{mpcdc2021safety} incorporates future states by coupling control objectives and saturation constraints with a discrete-time CBF constraint in an optimal control problem (OCP). However, the choice of the MPC horizon depends on real-time computational constraints, which can result in suboptimal performance.

% In this paper, we propose a LCA consisting of an offline library of nominal controllers and apply recent results from~\cite{o2013splitting, sindhwani2017sequential, srikanthan2023augmented} to generate an offline library of long-horizon nominal controllers.   Each nominal controller is obtained by solving a constrained OCP using the ADMM algorithm to obtain a feedfoward term that brings the system to the target and a feedback gain matrix to stabilize the system locally around the nominal trajectory. The resulting trajectories cover the state space uniformly from the initial location to the target. To generate the library of nominal controllers, we do not assume access to a map or knowledge of obstacles. Trajectory selection is carried out online by a nearest neighbor search over predicted next states from the collection of nominal controllers. Once the nominal input is selected, we solve a quadratic program with a CBF constraint to obtain an input that minimally deviates from the nominal input to guarantee safety. Therefore, our contributions are as follows
% \begin{enumerate}
%     \item To achieve real-time performance while ensuring task completion, we propose a layered solution that consists of a library of nominal controllers in the top layer, a trajectory selector in the middle layer, and a reactive safety filter in the lowest layer.
%     \item Each nominal controller is computed offline via ADMM and consists of a feedforward term that brings the system to the target and a feedback gain matrix to stabilize the system locally around the nominal trajectory.
%     \item Trajectory selection using a nearest neighbor search over predicted feasible next states and obstacle avoidance via control barrier functions are carried out online satisfying real-time computational guarantees and safety.
%     \item We provide an open-source implementation of our approach and tools to specify hyperparameters to ensure the generation of compliant policies.
% \end{enumerate}

% we use recent results from that exploit the structure of ADMM to design a fast solver for OCPs to 


% Several prior works from the robotics community show how to obtain ``full-stack'' safety/stability/performance guarantees for such layered architectures, see for example~\cite{rosolia2020multi,csomay2022multi,rosolia2022unified,garg2021multi}, by appropriately constraining planned trajectories to account for feedback control tracking error.  In addition, work from formal methods solving discrete planning problems over continuous dynamics can be viewed as a layered approach, to solving a complementary planning and control problem~\cite{lindemann2018control,dimitrova2014deductive,raman2014model,sadraddini2015robust,wolff2014optimization,wolff2012robust,fan2020fast,kress2009temporal}. 



% However, the question of safety while satisfying recursive feasibility in dynamic environments where only nearby obstacle locations are known is unanswered. To address this question, prior work called MPC-CBF~\cite{mpcdc2021safety} incorporates future states by coupling control objectives and saturation constraints with a discrete-time CBF constraint in an optimal control problem (OCP) to ensure safety. However, the choice of the MPC horizon depends on real-time computational constraints, which can result in suboptimal performance for very short horizons. 

% Recent work from~\cite{mpcdc2021safety} designs a MPC algorithm by solving an OCP  with a discrete-time control barrier function (CBF) constraint to guarantee safety. Although their approach is no longer reactive, the choice of MPC horizon is largely governed by the computation time required for real-time operation. In many cases, this choice leads to very short horizons and suboptimal performance. Moreover, their approach assumes knowledge of obstacles or a map to guarantee safety. 

% A recent survey~\cite{matni2024towards} of layered control architectures (LCAs) describe the mathematical principles governing the burgeoning success of LCAs for robotic systems through optimization relaxations. To obtain a LCA, a relaxation is applied to OCPs with complex dynamics, saturation, and obstacle avoidance constraints to obtain individual OCP that either consider obstacles or dynamics. For example, RRT~\cite{} coupled with a PD controller is an example of a LCA. Several prior works~\cite{}


% Inspired by the burgeoning success of layered control architectures (LCA)~\cite{matni2024towards, rosolia2022unified} for robot planning and control, we propose a LCA that consists of three layers; a library of nominal controllers in the top layer, a trajectory selector in the middle layer, and a reactive safety filter in the lowest layer.

% Reactive obstacle avoidance methods such as control barrier function (CBF) based safety filters do not account for future states due to the computation time needed for real-time operation. Prior work studies the use of model predictive control (MPC) over short horizons coupled with a discrete-time CBF constraint (MPC-CBF) to guarantee safety. However, the choice of MPC horizon in order to satisfy real-time computational constraints results in suboptimal performance in practice. In this paper, we consider the problem of navigation in an unknown environment for a robot equipped with a LiDAR sensor for real-time obstacle detection. To achieve real-time performance while staying feasible with respect to actuator limits, we propose a layered solution that consists of a library of nominal controllers in the top layer, a trajectory selector in the middle layer, and a reactive safety filter in the lowest layer. Each nominal controller is computed offline by solving a constrained optimal control problem (OCP) using the alternating direction method of multipliers (ADMM) algorithm to obtain a feedfoward term that brings the system to the target and a feedback gain matrix to stabilize the system locally around the nominal trajectory. The resulting trajectories cover the state space uniformly from the initial location to the target. Trajectory selection is carried out online by a nearest neighbor search over predicted next states from the collection of nominal controllers. Once the nominal input is selected, we solve a quadratic program with a CBF constraint to obtain an input that minimally deviates from the nominal input to guarantee safety. We show empirical evaluations on numerical simulations for a cartpole, unicycle and a Dubins car dynamics model in complex obstacle environments and compare against MPC-CBF and an ablative baseline CBF-QP that do not consider future predictions. Further, we evaluate our proposed layered solution on a Fetch --- and find that our method outperforms both baselines. 

% Ensuring the safety of the robot and its surroundings is critical in navigation tasks, adding another layer of complexity. Finally, effective navigation often requires the integration of perception algorithms to perceive the environment and make decisions based on the perceived information, further complicating the control problem. Overall, these factors contribute to making robot navigation a hard control problem that requires advanced algorithms and techniques to achieve reliable and efficient navigation in real-world environments.

% \yifan{rewrite based on motivation from input constraints} 
% Prior work on nonlinear model predictive control guarantees constraint satisfaction, however, they have a high computational burden when applied to high-dimensional continuous state and action spaces. Moreover, in the presence of dynamic obstacles assuming complete information of changes in the environment becomes an unreasonable assumption. For such scenarios, real-time controllers synthesized by solving a quadratic program (QP) with a control barrier function (CBF) constraint are a useful alternative. Still, control barrier functions designed for high-order dynamics systems lack global vision as a trade-off to reactivity and are therefore stuck in infeasible conditions from time to time under input constraints. 

% designing a nominal controller satisfying input constraints followed by feedback control design.

% A drawback of synthesizing a controller using CBF-QPs is the lack of global convergence guarantees to a goal for nonlinear systems due to the existence of local minima. \textcolor{red}{Need to verify} \yifan{move by cbf with lca discussion here}

% Therefore, to design controllers that handle input constraints while also accounting for real-time changes in the environment such as moving obstacles, we propose a layered control architecture. 

% Here, we propose to resolve the infeasibility issue encountered by CBF in high-order dynamics systems by designing a nominal controller with a feedback component that can enforce input constraints approximately. The layered approach gives you the flexibility to shift input constraints from the CBF to the nominal control design. For example, a two-layered architecture is composed of a top layer that computes a nominal controller with a reduced order discrete-time model $\Bar{f}$ over a long horizon and a low layer that applies a tracking controller for the nonlinear system $f_d$ over a short horizon. In the next section, we show how to derive a layered control architecture from a nonlinear optimal control problem and discuss its application to differential drive robot navigation.




%trajectory generation designs a desired reference assuming certain system properties. For example, prior work~\cite{todorov2005generalized} proposed the design of desired reference trajectories as the iterates from previous linearizations of the nonlinear system. However, this method highly depends on the initialization of the desired reference. Another example of trajectory generation assumes system-level properties such as differential flatness~\cite{murray2009optimization} which decouples the flat outputs that specify the trajectory. Although such decompositions have made a significant impact in various sub-fields, there is no existing theory establishing the mathematical principles behind the design of such layers for nonlinear optimal control. More recently, there has been a shift towards the design of hierarchical schemes termed as planner-tracker frameworks \cite{tedrake2010lqr, rosolia2020multi, herbert2017fastrack, schweidel2023safe} especially useful in navigation systems. The emphasis of such methods is on safety and fast online computation and hence, solves trajectory generation as a top-layer long horizon planning problem with a reduced order dynamics model running at lower frequencies and low-layer reactive tracking controller with a high-fidelity dynamics model running at higher frequencies. However, such approaches do not describe how the model mismatch between the different layers could plan infeasible reference trajectories when there are unbounded disturbances or for unstable systems.

%Although such decompositions have made a significant impact in various sub-fields, there is no existing theory establishing the need for designing components or layers such as trajectory generation and tracking control for nonlinear optimal control. For the disturbance setting, there have been several attempts in robust control, the most notable of which is tube-based MPC for bounded disturbances in both linear \cite{langson2004robust} and nonlinear settings \cite{kogel2015discrete}. Prior work on nonlinear optimal control \cite{todorov2005generalized} solves for locally convex approximations by linearizing around a nominal trajectory. This leads to a locally optimal feedback controller. 

% \emph{Paper organization:} 
% We show how ADMM applied to an optimal control problem results in a layered control architecture in Section~\ref{sec:prelims}. In Section~\ref{sec:method}, we instantiate our layered control architecture in the context of a deterministic and stochastic linear system. In Section~\ref{sec:non-lin}, we discuss extensions to the nonlinear setting.  We evaluate our proposed approach in several numerical examples in Section~\ref{sec:sim}, and end with conclusions and future work in Section~\ref{sec:conclusion}.

==> tex/2-Related-Work.tex <==
\section{Related Work}\label{sec:related-work}
We discuss related work on two degree of freedom (2DOF) architectures and LCAs to motivate the use of the alternating direction method of multipliers (ADMM) algorithm for path generation. We also provide an overview of reactive methods for obstacle avoidance to motivate the use of MCBF. 

\subsection{2DOF and Layered Control Architectures} 
In linear control systems, the term 2DOF controllers refer to control laws that consist of a feedforward term, which drives the system to the desired trajectory, and a feedback term to compensate for errors~\cite{murray2009optimization}.  Analogous design patterns are observed in robust MPC.  For example, tube-based MPC approaches broadly apply a control input of the form $u = K(x-x_d) + u_d$, where $(x_d,u_d)$ are nominal state and control inputs computed by solving an optimization problem online, and $K(x-x_d)$ is a feedback term compensating for errors between the actual system state $x$ and the reference state $x_d$. For nonlinear systems, trajectory generation and feedback control are typically decoupled, although approaches exist that do not explicitly make this separation, e.g., iLQR~\cite{todorov2005generalized}.  
% A typical design pattern consists of generating a(n) (approximately) dynamically feasible and safe reference trajectory, e.g., by exploiting differential flatness or a reduced order model, and then applying locally stabilizing feedback control to ensure trajectory tracking, e.g., via linearization or control Lyapunov functions~\cite{galloway2015torque}. 
In this paper, we exploit the structure of ADMM applied to optimal control problems (OCP)~\cite{srikanthan2023augmented} to obtain a 2DOF controller with a feedforward term and feedback gains. We use the time-varying feedback gain matrices online to locally stabilize the system whenever the robot switches from one path to the next due to the presence of an obstacle. 

\subsection{Reactive methods for Obstacle Avoidance}
Collision-free guarantees in dynamic environments are achieved either through the satisfaction of constraints in optimization-based approaches \cite{ames2019control,mpcdc2021safety,9653152,9319250,8967981,10380695} or through reactive potential-field inspired closed-form solutions \cite{apf1989real,navigationf1992exact,harmonic1997real,khansari2012dynamical,6907685,LukesDS,billard2022learning,10164805}.  Among all methods, only CBF-QP~\cite{ames2019control} can minimize deviations from nominal controller behavior while ensuring safety for general control-affine systems and a general class of obstacle geometries~\cite{blanchini2015invariant}. While methods to enforce robot input constraints optimally for Dynamical System motion policy modulation (Mod-DS) are proposed in \cite{xue2024nominima}, its applications are limited to fully actuated systems. Although variants of CBF-QP, such as CBF-CLF-QP are available for safe reactive navigation tasks without the use of a nominal controller, designing the Control Lyapunov Function (CLF) for navigation tasks in general is challenging and not the focus of this work. In this paper, we generate feasible paths offline to alleviate the need for enforcing tight input constraints online and guide the robot to the goal while maintaining safety through reactive methods.

%In the following section, we formalize our problem and provide the necessary background to introduce our method.
% \subsection{Notation}
%
%MPC is a receding-horizon control method to provide optimal solutions for linear systems in finite horizon settings in the presence of state and input constraints \cite{morari1999model} with extensions to disturbance settings~\cite{langson2004robust, kogel2015discrete}. In robust MPC, in particular, tube-based MPC, the two degree of freedom design becomes apparent where the feedback term comes from the error dynamics and the feed forward term brings the system to a desired state.
%



==> tex/3-Background.tex <==
\section{Background and Problem Formulation}\label{sec:prob-form}
Consider a continuous-time control-affine nonlinear system of the form 
\begin{equation}\label{eq:ct-sys}
    \dot{x}(t) = f(x(t)) + g(x(t))u(t)
\end{equation}
where $t, t_f \in \R$ are continuous-time parameters with $t$ ranging from $0$ to $t_f$, $x(t) \in \R^n$ is a state vector, $u(t) \in \R^m$ is a control input vector, and $f:\R^n \to \R^n$, and $g:\R^n\to \R^{n \times m}$ define the control-affine nonlinear dynamics. %\rev{We denote the space of real numbers by $\R$ and states evolving on the unit-sphere manifolds by $\mathbb{S}$.} 
Our objective is to design $u(t)$ to bring the system~\eqref{eq:ct-sys} from initial state $x(0)=\xi$ to goal state $x(t_f)=\xi_g$ while remaining safe and satisfying input constraints, i.e., $u(t) \in \calU$ where 
\begin{equation}\label{eq:input-const}
    \calU = \{u \in \R^m\ |\ u_{\min} \leq u \leq u_{\max}\}.
\end{equation}

We define the notion of robot safety and consider safe control algorithms based on boundary functions. Given a twice-differentiable function $h_j$ for each obstacle $j \in \calO_{x, t}$ where $\calO_{x, t}$ denotes the set of visible obstacle indices, we define a safe set with boundary function $h_j:\R^{n} \times \R^{p} \rightarrow \R$ as the following,
\begin{equation}~\label{eq:safe-region}
    \calC = \{x \in \R^{n} \  |\ h_j(x, x_\text{o}^j(t)) > 0, \ \forall j \in \calO_{x,t},\ t \in [0, t_f]\},
\end{equation}
where $x_\text{o}^j$ is the instantaneous obstacle state including its position and orientation and $p$ is the obstacle state dimension.
% When obstacles are static, the safe set $\calC$ is fully determined by the robot state and obstacle states in its local radius. When obstacles are moving, we require obstacle velocities as well to determine $\calO_{x, t}$. 
% We abuse notation here to define the visible obstacle indices ($\calO_{x, t}$) as a function of robot state and time, however, note that they do not explicitly depend on time. They are determined by the instantaneous position and orientation of moving obstacles.
% In future work, we aim to provide a rigorous characterization of safe sets for moving obstacles with arbitrary geometries.}

% Given a continuously differentiable function \rev{$h_j$ for each obstacle $j \in \calO_t$ where $\calO_t$ is the set indices of visible obstacles at time $t$}, we define \rev{a time-varying} safe set with boundary function $\rev{h_j}:\R \times \R^n \rightarrow \R$ as
% \begin{equation}~\label{eq:safe-region}
%     C_t = \{x \in \R^n\ |\ h_j(t, x) > 0, \ \forall j \in \calO_t\}.
% \end{equation}
% % Here, $C_t$ is outside, $\partial C_t$ lies on the boundary with $h(t, x) = 0$, and the unsafe set $\neg C_t$ is inside the visible obstacles with $h(t, x) < 0$. 
% \rev{For example, a moving circular obstacle has a boundary function of the form
% \begin{equation*}
%     h(t, x) = \|x - x_c(t) \|_2^2 - c_r^2
% \end{equation*}
% where $x_c(t), c_r$ are the center and radius of the obstacle, and $h(t, x) > 0$ implies that $x$ lies outside the obstacle boundary. For arbitrary shaped obstacles and partial boundaries in the field of view, we represent the boundaries using Gaussian Process based distance functions following prior work~\cite{choi2024towards}. For more details, refer to our arxiv version appendix details. TBD.}
% In environments with dynamic obstacles, the safe sets $C$ vary with both time and state. In scenarios with static obstacles, $C$ varies only with state and the boundary function $h$ is given by $h(t, x) = h(0, x),\ \forall t$. When the robot is at state $x(t_0)$, we assume that we have access $h(t_0, x)$ (i.e., the robot knows the boundaries of nearby obstacles). 
% and no knowledge of future boundary functions. 

Given the above definitions, we formulate an optimal control problem (OCP) with an objective function $J$ as
\begin{equation}\label{prob:ct-ocp}
    \begin{array}{rl}
         \mathrm{minimize} &\int_{0}^{t_f} J(x(t), u(t))\\
        \mathrm{subject\ to } & \dot{x}(t) = f(x(t)) + g(x(t))u(t), \ t \geq 0, \\
        &u(t) \in \calU, \ t \geq 0, \\
        & x(t) \in \calC,
        % & \nabla_{x, x_o^j} h_j(x(t), x_\text{o}^j(t)) > 0, \ \forall j \in \calO_{x, t},
        % & \dot{h}_j(t, x(t)) \geq 0, \ \forall j \in \calO_t
        % & x(t) \in C_t,\ \forall t \geq 0, 
    \end{array}
\end{equation}
while satisfying boundary conditions given by $x(0) = \xi$ and $x(t_f) = \xi_g$. The problem in~\eqref{prob:ct-ocp} poses three challenges: a) input constraint satisfaction, b) safety, and c) real-time computation. To handle safety and real-time computation, prior work~\cite{ames2019control, loizou2007mixed, loizou2003closed} design reactive controllers to maintain the state within a time-invariant safe set. 
% However, such reactive methods suffer from local minima or limit cycles preventing their use for long-horizon tasks. 
Recent work~\cite{mpcdc2021safety, liu2024safety} tackles input constraint satisfaction and safety by using MPC to solve a discrete-time version of~\eqref{prob:ct-ocp}. In practice, nonlinear MPC suffers from computational burden and solver infeasibility for long-horizon problems. 
% The guarantee in discrete-time does not translate to robot safety if the solver is infeasible or doesn't finish computation within the frequency of operation. 
Several works~\cite{rosolia2022unified, grandia2021multi} attempt to tackle all three challenges through LCAs running low-frequency MPC without safety constraints at the higher layer and CBF-QP at the lower layer. However, without careful coordination between the layers, we empirically observe that such approaches i) still suffer from local minima in cluttered environments with concave obstacles and ii) may lead to infeasible solutions for control-affine systems with tight input constraints ($u(t) \in \calU$). 
% $u(t)\in[u_{\min},u_{\max}]$. 

\emph{Problem Statement}: To address the combined problem of input feasibility, safety and real-time computation in~\eqref{prob:ct-ocp}, we consider the design of offline long-horizon path planners, accompanied by fast online feedback solvers and an appropriate reactive strategy to ensure safety and task completion.

% Therefore, recent attention towards designing LCAs~\cite{matni2024towards, rosolia2022unified, rosolia2020multi} wherein 

% In practice, $h(t, x)$ is often measured as the distance from the controlled agent to the obstacle surface boundary. The goal of a safety-critical controller is to generate an input $u$ that maintains the state of the DS $x$ within the safe set $C$ while converging to a target $x^* \subset C \in\mathbb{R}^n$.

% and $f, g$ are derived from the mechanical dissipativity or Euler-Lagrange equations of the system. 
% Our objective is to design a feedback controller that satisfies real-time computational performance guarantees while ensuring safety to bring the system from an initial state $\xi$ to a goal state $\xi_g$. Next, we provide our definitions of safety introducing CBFs using boundary functions for obstacle avoidance.

% \textbf{NIK: it would be useful to pose the nominal control problem formally here (in terms of taking state from $\xi$ to $\xi_g$ in time $T$), and define its solution as the nominal controller.  Then the MCBF-QP approach below can be posed properly.  We are relying too much on the nebulous term ``nominal controller'' throughout the intro and this section.}

% \yifan{This subsection needs fixing. I'm not sure of the math for MCBF. Please fill me. No need to introduce CBF-QPs I think, since it is standard and they can read Aaron's work.}
% \subsection{Safety via CBFs and Obstacle Definition}
% We define the notion of robot safety and generate safe control algorithms based on boundary functions. Given a continuously differentiable function $h$, state $x \in \mathbb{R}^n$, and continuous time parameter $t \in \mathbb{R}$, $h:\mathbb{R}^n \rightarrow \mathbb{R}$ is a boundary function~\cite{ames2019control} if the safe set satisfies
% \begin{equation}
% C=\{x \in \mathbb{R}^n: h(x,t)>0\}.\label{safe region}
% \end{equation}
% Here, $C$ is outside the obstacle, $\partial C$ lies on the boundary of the obstacle with $h(x,t) = 0$, and the unsafe set $\neg C$ is inside the obstacles with $h(x, t) < 0$. 
% of the system can be defined as in \eqref{safe region},\eqref{boundary},\eqref{unsafe region}\cite{ames2019control}. 
% The boundary function $h$ is time-dependent for scenarios where the unsafe sets are moving while static obstacles have a boundary function given by $h(x,t)=h(x)$. 
% \begin{equation}
% \partial C=\{x \in \mathbb{R}^n: h(x,t)=0\}\label{boundary}
% \end{equation}
% \begin{equation}
% \neg C=\{x \in \mathbb{R}^n: h(x,t)<0\}\label{unsafe region}
% \end{equation}
% In practice, $h(x,t)$ is often measured as the distance from the controlled agent to the obstacle surface boundary. The goal of a safety-critical controller is to generate an input $u$ that maintains the state of the DS $x$ within the safe set $C$ while converging to a target $x^* \subset C \in\mathbb{R}^n$.

% \subsection{Brief introduction of CBFs}
% To tackle this problem, CBF-QP minimally adjusts a nominal controller while ensuring safety through affine inequality constraints in the context of set invariance~\cite{ames2019control}. In CBF formulation, the boundary function $h(x,t)$ is called the barrier function. To guarantee that the controlled agent will never step outside the safe set $C$, 
% % $C=\{x \in \mathbb{R}^n: h(x,t)>0\}$, 
% CBF-QP utilizes barrier functions to ensure set invariance of $C$ when solving the optimization problem. 
% Given control affine systems defined in \eqref{eq:ct-sys}, standard CBF-QP solvers are formulated as the following quadratic program 
% \begin{gather}
% \nonumber u_{\text{cbf}} = \argmin_{{u} \in \mathbb{R}^p}\frac{1}{2}||u-u_{\text{nom}}||^2\\
% \Dot{h}(x,u,t) =L_fh(x,t) + L_gh(x,t)u + \frac{\partial h(x,t)}{\partial t}\geq -\alpha (h(x,t))
% \label{eq:cbf-qp affine} 
% \end{gather}
% where $u_{\text{nom}}$ is a nominal control input, $L_f$ is a lie-derivative \yifan{fill me}. 
% Throughout the rest of the paper, we model the safe set using boundary functions.

% However, a major drawback of using the standard CBF-QP is the existence of local minima, and even trapping regions in concave obstacle environments from the resulting trajectories. Entering a local minimum state will deteriorate robot's task performance by preventing it from converging to the target states. Recent work~\cite{} \yifan{fill me with on manifold description} Nevertheless, when robot model uncertainties and environmental noises are involved, even on-Manifold CBF-QP's performance could lead to limit cycles when infeasible nominal controllers are designed from greedy policies.

% \subsection{Optimal control problem}
% To this end, we consider a discrete-time nonlinear system obtained by the Runge-Kutta discretization of~\eqref{eq:ct-sys} with a sampling time of $T_s$ seconds as
% \begin{equation}\label{eq:nonlin-sys}
%     x_{i+1} = f_d(x_i, u_i)
% \end{equation}
% where $f_d$ is the discretized dynamics, $x_i \in \R^n$ is a state vector and $u_i \in \R^m$ is a control input vector at time $i$. We want to design a controller such that the input satisfies saturation constraints given by $u_i \in \calU$ where $\calU = \{u \in \R^m\ |\ u_{\min} \leq u_i \leq u_{\max}\}$ such that $u_{\min}, u_{\max}$ are lower and upper limits and states satisfy $x_i \in C_i$ where $C_i$ are safe sets defined using boundary functions that change over time as new obstacles are detected online. The initial safe set $C_0$ is assumed to be known. Our objective is to design a controller that is fast to compute to bring the system~\eqref{eq:nonlin-sys} from an initial location to a goal, while staying feasible in both states and inputs. We pose this as a discrete-time OCP over a horizon $T$ given by
% \begin{equation}\label{prob:global-ocp}
%     \begin{array}{rl}
%         \mathrm{minimize} &\sum_{i=0}^{T-1} J_i(x_i, u_i) + J_T(x_T - \xi_g) \\
%         \mathrm{subject\ to } & x_{i+1} = f_d(x_i, u_i), \ i \geq 0, \\
%         & x_i \in C_i, \quad u_i \in \calU, \ i \geq 0, \\
%         & x_0 = \xi,
%     \end{array}
% \end{equation}
% where $J_i$ is a stage cost function and $J_T$ is a terminal cost function. 



% We make the following assumptions to guarantee the existence of a local optimum.

% \begin{assumption}\label{assum:convexity-diff}
%     The (extended-real-valued) functions $J_i: \R^{n+m} \rightarrow \mathbb{R} \cup \{+\infty\}$, and $J_T: \mathbb{R}^n \rightarrow \mathbb{R} \cup \{+\infty\}$ are closed, proper, and convex. The dynamics $f_d \colon \R^{m+n} \rightarrow \R^n$ is differentiable. 
% \end{assumption}

% \begin{assumption}\label{assum:lagrangian}
%     The standard Lagrangian for problem~\eqref{prob:global-ocp} has a saddle point. 
% \end{assumption}

==> tex/4a-AugmentedLCA.tex <==
\section{ADMM-MCBF as a Layered Control Architecture}
\label{sec:admm-cbf-lca}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{img/front_and_back_nom_traj_new.png}
%     \caption{We show a plot of }
%     \label{fig:multi-path-admm}
% \end{figure}
% We do not assume knowledge of obstacle locations but instead use a sensor to detect boundaries within the field of view online.
Our goal is to design a long-horizon path planner to guide the system to a goal state, while leveraging reactive policies to ensure safety. To this end, we propose a layered solution that consists of an offline path planner used to generate a feasible path library, an online path selector, and an online safety filter as shown in Figure~\ref{fig:intro-block-diag}. 
% For path library generation, we apply recent results from~\cite{o2013splitting, sindhwani2017sequential, srikanthan2023augmented} using the alternating direction method of multipliers (ADMM) algorithm to efficiently solve constrained OCPs. 
The feasible path library provides controllers, reference trajectories, and time-varying feedback gain matrices to stabilize the system locally around the generated trajectories. Moreover, these gains allow for a smooth proportional control action whenever the robot transitions between paths if the robot is near an obstacle.
% In this paper, we empirically illustrate the tradeoff between incorporating constraints or lack thereof at different layers.}
% generate feasible long-horizon controllers in a computationally efficient manner. Each nominal controller is obtained by solving a constrained optimal control problem (OCP) using the ADMM algorithm. 
% A benefit of using ADMM gives us instantaneous access to time-varying feedback gain matrices during online execution. 
% is approach is that we obtain an analytical closed-form for the time-varying feedback gain matrices for the entire horizon due to sequential linearization. 

% The \rev{trajectories in the path library are optimized by carefully sampling waypoints}, as shown in Figure~\ref{fig:multi-path-admm} and described in the next subsection, from the initial location to the goal. To perform path selection online, we use a nearest neighbor search over predicted next states from the collection of paths. Once the path is selected, we compute the nominal feedback control input and solve a quadratic program with a MCBF constraint to obtain a safe input that minimally deviates from the nominal input.

% Stable dynamic systems are popular in fully-actuated robot applications for their ability in consistently directing the robot towards the goal states even when the control agent deviates from its origin trajectory. The limitation of dynamics systems, however, is their incapability of enforcing robot actuation limits in the design process. For nonholonomic robots, like the commonly used differential drive systems, reaching goal state convergence using closed-form dynamic systems is nearly impossible. In the construction of our multi-trajectory nominal control system, we mimic the characteristics of stable dynamic systems to cover the exploration areas with evenly distributed input and kinematic feasible trajectories. To ensure clean and even distribution of the generated trajectories, we introduce a reasonable number of waypoint constraints during the nominal controller computation. Having clean and evenly distributed trajectories in the nominal controller system makes it easier for the robot to navigate from one to another using methods detailed in \autoref{sec: nom fd controller}.

\subsection{Offline Feasible Path Library Generation}
\subsubsection{Waypoint generation}
The trajectories associated with each path in the path library are regulated by two user-design choices: the inter-trajectory intervals $\delta$, and the number of waypoints per trajectory $\tau$. We assume that the users have access to the approximate size of the exploration field, i.e., how large an area the robot explores to complete a task (e.g., reaching a goal). For example, given a room of width $L$, we generate $N=L/\delta$ offline paths. We choose $\delta$ sufficiently small to provide the robot with the flexibility to avoid getting trapped. 
% For most of the scenarios we consider, generating waypoints in the rectangle of dimensions $L$ by $N\delta$ between $\xi$ and $\xi_g$ is sufficient (colored yellow in \autoref{fig:intro-block-diag}). In rare cases when the initial state is inside the exploration space and not at a boundary, we also manually generate points colored in orange as shown in \autoref{fig:intro-block-diag}.
For most of the scenarios we consider, we grid sample a fixed number of points along the direction towards the goal dispersed by $\delta$ (colored yellow in \autoref{fig:intro-block-diag}). In other scenarios where trajectories evolve away from the goal, we sample points (colored in orange in~\autoref{fig:intro-block-diag}) by selecting some of them manually to improve optimization convergence of the algorithm in the following section.
% In future work, we aim to formally characterize how the choice of samples relates to convergence. 

% waypoints are sampled from a grid of length $\delta$ and width $D/\tau$ where $D$ is the Euclidean distance between initial and goal $(x, y)$ position. Whenever trajectories are designed in the direction opposite to the goal, we manually select a few points to provide a more dense sampling of the space.
% grid sampling, in which points' distances with respect to each other along the length and the width of the grid are $\frac{D}{\tau}$ and $N$, where $D$ is the Euclidean distance between $\xi$'s position and $\xi_g$'s position. 

% In rare cases where the robot is surrounded by obstacles and needs to first move away from the target, we perform a similar grip sampling algorithm but manually modify some point locations to help offline path generation algorithms converge, as shown in orange points in \autoref{fig:intro-block-diag}. 
% is provided using similar algorithms with additional steps to sample a few more waypoints in $\vec{n}$ directions starting from $\xi$. 

% We present a pseudo-code in Algorithm~\ref{alg:waypoint-generation} for waypoint generation, where $W$ is the set of all waypoints, and $w_p(k)$ denotes the $k$th waypoint associated with path $p$. The vector $\vec{d}$ connects $\xi$ to $\xi_g$, and $\vec{n}$ is normal to $\vec{d}$. 
% Smaller $\delta$ values would result in a larger runtime, while large $\delta$ values may not provide enough paths for the robot  that are too large would cause the nominal controller input to be less realizable when shifting from one trajectory to the next. In practice, we found that our offline nominal controllers takes $N$ seconds or less but might also take up to $N$ minutes to finish computation depending on the problem specification. 
% However, using parallelized hardware implementation we can achieve a significant speedup.


% , where $\xi$ and $\xi_g$ is the initial and goal state of the robot, 
% For the algorithm block, $P_k$ with an integer $k$ the waypoint constraint sets for the $k$th nominal controller in the system, and $P$ is the complete set of waypoints used to generate the entire multi-trajectory system. In some cases, where the robot's initial location is surrounded by obstacles in the direction towards the goal location, and have to first detour and move away from the goal. In those cases, we provide the option to produce feasible trajectories first traveling in the opposite directions to make sure that the robot has access to feasible nominal inputs under all circumstances. Following the same naming convention, We denote the number of nominal trajectories that travel initially opposite to the goal as $N_b$, the number of waypoints in the detouring directions of the added trajectories $\tau_b$, and the number of waypoints in the non-detouring parts of the added trajectories $\tau_f$. In other words, the total number of waypoints in the added trajectories is $\tau_f + \tau_b$.

% Solving the OCP in~\eqref{prob:global-ocp} to convergence is computationally expensive and in our problem setting where only $C_0$ is known apriori, it is impossible without further assumptions. Therefore, we assume that we have knowledge of the types of boundaries that the robot will encounter during its exploration and that it is equipped with a short range sensor that can detect the boundaries of nearby obstacles. 
% We note here that our goal is not to create a map of our environment but to safely navigate the robot from the initial location to the goal while respecting computational constraints.

% $W = \{\{w_p(k)\}_{k=1}^{\tau}\}_{p=1}^{N}$

% \begin{algorithm}
% \footnotesize
% \caption{Waypoint Generation}\label{alg:waypoint-generation}
% \begin{algorithmic}
% \Inputs{$\xi, \xi_g, \delta,N, \tau$}
% \Initialize{$W \gets \emptyset$}
% % \State{$W_1, W_2,\ldots,W_N \gets \emptyset$}
% \State $\Vec{d}= \xi_g-\xi,\quad \Vec{n}\perp \vec{d}$
% \State $\text{mid} \gets \text{int}(\frac{N+1}{2})$
% \For {$k=1,2,\ldots, \tau$}
% \State $w_\text{mid}(k) \gets \xi_0+\frac{k\Vec{d}}{\tau+1}$
% % \State $W_\text{mid}.\text{insert}(w_\text{mid}(k)) $
% \For {$j=1,2,\ldots, \text{mid}$}
%     \State $w_{\text{mid}+j}(k) = w_\text{mid}(k)+\delta j \vec{n}$
%     \State $w_{\text{mid}-j}(k) = w_\text{mid}(k)-\delta j \vec{n}$
%     % \State $W_{\text{midI}+j}.\text{insert}(w_{\text{midI}+j}(k)) $
%     % \State $W_{\text{midI}-j}.\text{insert}(w_{\text{midI}-j}(k)) $
% \EndFor

% % \For {$p=1,2,\ldots, N$}
% %     \State $W.\text{insert}(W_p) $
% % \EndFor
% \EndFor
% \State \Return $W =\{\{w_p(k)\}_{k=1}^{\tau}\}_{p=1}^{N} $
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
% \footnotesize
% \caption{Waypoint Generation}\label{alg:waypoint-generation}
% \begin{algorithmic}
% \Inputs{$\xi, \xi_g, \delta,N, \tau, \text{backCoverage}, N_\text{b}, \tau_\text{b}, \tau_\text{f}$}
% \Initialize{$P, P_1, \ldots,P_N,\ldots, P_{N+2N_b} \gets \emptyset$}
% \State $\Vec{d}= \xi_g-\xi_0,\quad \Vec{n}\perp \vec{d}$
% % \Comment{Construct normalized vector $\vec{n}$ s.t. $\vec{n}$ is perpendicular to the linear trajectory connecting $\xi_0, \xi_g$.}
% \State $\text{midI} \gets \text{int}(\frac{N+1}{2})$
% \For {$i=1,2,\ldots, \tau$}
% \State $\text{midP} \gets \xi_0+\frac{i\Vec{d}}{\tau+1}$
% \State $P_\text{midI}.\text{insert}(\text{midP}) $
% \For {$j=1,2,\ldots, \text{midI}$}
%     \State $P_{\text{midI}+j}.\text{insert}(\text{midP}+\delta j \vec{n}) $
%     \State $P_{\text{midI}-j}.\text{insert}(\text{midP}-\delta j \vec{n}) $
% \EndFor
% \EndFor
% \If{not backCoverage}
% \State \Return $P =[P_1,P_2,\ldots,P_n]$
% \Else
% % \State $\text{midI} \gets \text{int}(N+1)$
% \For {$i=1,2,\ldots, \tau_b$}
% \State $\text{iniP}_1 \gets \xi_0-\delta i\Vec{n}$
% \State $\text{iniP}_2 \gets \xi_0+\delta i\Vec{n}$
% \State $P_\text{N+1}.\text{insert}(\text{iniP}_1) $
% \State $P_\text{N+1}.\text{insert}(\text{iniP}_2) $
% \For {$j=2,\ldots, N_b$}
%     \State $P_{N+2j-1}.\text{insert}(\text{midP}+\delta j \vec{n}) $
%     \State $P_{N+2j}.\text{insert}(\text{midP}-\delta j \vec{n}) $
% \EndFor
% \EndFor

% \For {$j=1,\ldots, N_b$}
%     \State $P_{N+2j-1}.\text{stack}(P_0[-\tau_f:]) $
%     \State $P_{N+2j}.\text{stack}(P_N[-\tau_f:]) $
% \EndFor
% \State \Return $P =[P_1,P_2,\ldots,P_{N+2N_b}]$
% \EndIf
% \end{algorithmic}
% \end{algorithm}

% In what follows, we describe how we generate long-horizon path planners in a fast and efficient way that satisfies waypoint and input constraints.

% Therefore, we propose a relaxation that layers problem in~\eqref{prob:global-ocp} 
% To generate $N$ nominal controllers that are indexed by $p \in \mathbb{N}_+$, 

% we assume that $C_0$ is the safe set for our optimization and approximate it by selecting a sparse set of $N$ evenly spaced samples at fixed intervals $\delta$ where $\delta \in \mathbb{N}_+$ with a total of $\tau = \lf \frac{T}{\delta} \rf$ intervals. For each nominal controller $p$, the $\tau - 1$ samples at intervals of $\delta$ are denoted by $s(\lf \calT/\delta \rf, p)$ where $\calT = \{\delta, \cdots, (\tau - 1)\delta\}$ . 
% Here, $N$ is the total number of nominal controllers and $p$ is an index that refers a particular one.

% For example, choosing $T=40$ seconds and $\delta = 5$ seconds results in $\tau=8$ fixed intervals and $7$ waypoints between the initial location and the target. Given $N = 10$, we generate each nominal controller with their associated $7$ waypoints by including them as constraints in the optimization problem below (see Figure~\ref{fig:intro-block-diag} for clarity).

\subsubsection{Nominal Controller Design}
\label{sec: offline nom design}
To design $N$ input feasible feedback controllers such that their resulting trajectories satisfy the generated waypoints, we consider a discrete-time nonlinear system obtained by the Runge-Kutta discretization of~\eqref{eq:ct-sys} with a sampling time of $T_s$ seconds as
\begin{equation}\label{eq:nonlin-sys}
    x_{i+1} = f_d(x_i, u_i)
\end{equation}
where $f_d$ is the discretized dynamics, $x_i \in \R^n$ is a state vector and $u_i \in \R^m$ is a control input vector at discrete time step $i$. Our objective is to design discrete-time feedback controllers over a finite horizon $T$ such that the input satisfies saturation constraints given by $u_i \in \calU$. We do not consider safety constraints in this design step.
% where $\calU = \{u \in \R^m\ |\ u_{\min} \leq u_i \leq u_{\max}\}$ where $u_{\min}, u_{\max}$ are lower and upper limits, respectively. 

Let $T/(\tau+1) = \Delta$ such that $\Delta$ is divisible by $T_s$ and the time indices at which waypoint constraints are enforced be $\calT = \{\Delta, 2\Delta, \cdots, \tau \Delta\}$. The problem is succinctly described as the following constrained OCP solved for each nominal controller indexed by $p$ as
\begin{equation}\label{prob:library-ocp}
    \begin{array}{rl}
         \mathrm{minimize} &\sum_{i=0}^{T-1} J_i(x_{i, p}, u_{i, p})\\
        \mathrm{subject\ to } & x_{i+1, p} = f_d(x_{i, p}, u_{i, p}), u_{i, p} \in \calU, \ i \geq 0, \\
        & x_{0, p} = \xi, \ x_{T} = \xi_g, \\
        & x_{i, p} = w_p(\lf i/\Delta\rf), \forall i \in \calT, 
        % & r_{i, p} = x_{i, p},\ a_{i, p} = u_{i, p}
    \end{array}
\end{equation}
where $J_i$ are stage costs, and $w_p(\cdot)$ enumerates the generated waypoints for controller $p$. To solve problem~\eqref{prob:library-ocp}, we introduce redundant state and input equality constraints as in~\cite{srikanthan2023augmented} and apply the ADMM algorithm. To simplify notation, we drop references to indices $p$ and describe our algorithm for a single nominal controller. We note that computing the $N$ nominal controllers can be easily parallelized.% can compute $N$ controllers using parallel hardware to speed up the run time. 

For each nominal controller, define a state trajectory variable as $\boldsymbol{x}$, input trajectory variable as $\boldsymbol{u}$, and the combined trajectory variable as $\boldsymbol{z} = (\boldsymbol{x}^\top, \boldsymbol{u}^\top)^\top$. We introduce a redundant trajectory variable $\boldsymbol{\bar{z}}$ and an equality constraint $\boldsymbol{z} = \boldsymbol{\bar{z}}$ to optimization in~\eqref{prob:library-ocp}. Let $\boldsymbol{J}(\boldsymbol{\bar{z}}) = \sum_{i=0}^{T-1} J_i(\bar{z}_i)$, $\psi(\boldsymbol{z}; \xi) = \sum_{i=0}^{T-1}\psi(z_i, \xi)$ be a sum of indicator functions for dynamics constraints given as
\begin{equation*}
    \psi(z_i; \xi) = \begin{cases}
        0, & \text{if } x_{i+1, p} = f_d(x_{i, p}, u_{i, p}),\ \forall i > 0 \\
        0, & \text{if } \ x_{0, p} = \xi, i = 0 \\
        \infty, & \text{otherwise},
    \end{cases}
\end{equation*}
and $\bar{\psi}(\boldsymbol{\bar{z}}; w_p) = \sum_{i=0}^{T-1} \bar{\psi}(\bar{z}_i; w_p)$ be the sum of indicator functions for waypoints and input constraints defined as
\begin{equation*}
    \bar{\psi}(\bar{z}_i; w_p) = \begin{cases}
        0, & \text{if } i \in \calT,\  \bar{z}_{u, i} \in \calU, \text{ and } \bar{z}_{x, i} = w_p(i/\Delta), \\
        0, & \text{if } i \notin \calT,\ \bar{z}_{u, i} \in \calU, \bar{z}_{x,T} = \xi_g\\
        \infty, & \text{otherwise},
    \end{cases}
\end{equation*}
where $\bar{z}_{x,i}$ and $\bar{z}_{u, i}$ correspond to state and input redundant variables at time $i$, respectively.
% as $\boldsymbol{r_p}$ and $\boldsymbol{a_p}$, respectively. Let $z_p = (x_p^\top, $ Let the objective function be denoted by $\boldsymbol{J}(\boldsymbol{r_p}, \boldsymbol{a_p}; \xi_g) = \sum_{i=0}^{T-1} J_i(r_{i, p}, a_{i, p}) + J_T(r_{T, p}, \xi_g)$, the input box constraints by the set $\calU = \{ u \in \R^m\ |\ \underline{u} \leq u \leq \overline{u}\}$ and waypoint constraints at fixed intervals $\delta$ as an indicator function $\boldsymbol{\psi}(\boldsymbol{r_p}, \boldsymbol{s_p})$ such that 
% \begin{equation*}
%     \boldsymbol{\psi}(\boldsymbol{r_p, s_p}) = \begin{cases}
%         0, & \text{if } r_{\calT, p} = s(\lf \calT/\delta \rf, p),\\
%         \infty, & \text{otherwise}.
%     \end{cases}
% \end{equation*}
% Define $L_{\rho} (\boldsymbol{x_p}, \boldsymbol{r_p}, \boldsymbol{u_p}, \boldsymbol{a_p}, \boldsymbol{v_{r,p}}, \boldsymbol{v_{a,p}}) = \frac{\rho}{2} \left\Vert \begin{bmatrix}
%             \boldsymbol{x_p} - \boldsymbol{r_p} + \boldsymbol{v_{r,p}} \\
%               \boldsymbol{u_p} - \boldsymbol{a_p} + \boldsymbol{v_{a,p}}
%          \end{bmatrix} \right \Vert_2^2$
% To obtain the layered decomposition from~\cite{srikanthan2023augmented}, we apply the ADMM algorithm to~\eqref{prob:library-ocp} to get the following iterative updates as


% redundant variables $r_{i, p}$ for states, and $a_{i, p}$ for inputs by adding equality constraints to the optimization and generate a library of $N$ nominal controllers by solving
% \begin{equation}\label{prob:library-ocp}
%     \begin{array}{rl}
%          \mathrm{minimize} &\sum_{i=0}^{T-1} J_i(r_{i, p}, a_{i, p}) + J_T(r_{T, p}, \xi_g)\\
%         \mathrm{subject\ to } & x_{i+1, p} = f(x_{i, p}, u_{i, p}), \ i \geq 0,\ x_{0, p} = \xi, \\
%         & \underline{u} \leq a_{i, p} \leq \overline{u}, \ i \geq 0, \\
%         & r_{\calT, p} = s(\lf \calT/\delta \rf, p), \\
%         & r_{i, p} = x_{i, p},\ a_{i, p} = u_{i, p}
%     \end{array}
% \end{equation}
% where $p$ is the nominal controller index.

% For each nominal controller $p$, we define a state trajectory variable as $\boldsymbol{x_p}$, input trajectory variable as $\boldsymbol{u_p}$, redundant state and input trajectory variables as $\boldsymbol{r_p}$ and $\boldsymbol{a_p}$, respectively. Let $z_p = (x_p^\top, $ Let the objective function be denoted by $\boldsymbol{J}(\boldsymbol{r_p}, \boldsymbol{a_p}; \xi_g) = \sum_{i=0}^{T-1} J_i(r_{i, p}, a_{i, p}) + J_T(r_{T, p}, \xi_g)$, the input box constraints by the set $\calU = \{ u \in \R^m\ |\ \underline{u} \leq u \leq \overline{u}\}$ and waypoint constraints at fixed intervals $\delta$ as an indicator function $\boldsymbol{\psi}(\boldsymbol{r_p}, \boldsymbol{s_p})$ such that 
% \begin{equation*}
%     \boldsymbol{\psi}(\boldsymbol{r_p, s_p}) = \begin{cases}
%         0, & \text{if } r_{\calT, p} = s(\lf \calT/\delta \rf, p),\\
%         \infty, & \text{otherwise}.
%     \end{cases}
% \end{equation*}
% Define $L_{\rho} (\boldsymbol{x_p}, \boldsymbol{r_p}, \boldsymbol{u_p}, \boldsymbol{a_p}, \boldsymbol{v_{r,p}}, \boldsymbol{v_{a,p}}) = \frac{\rho}{2} \left\Vert \begin{bmatrix}
%             \boldsymbol{x_p} - \boldsymbol{r_p} + \boldsymbol{v_{r,p}} \\
%               \boldsymbol{u_p} - \boldsymbol{a_p} + \boldsymbol{v_{a,p}}
%          \end{bmatrix} \right \Vert_2^2$
To obtain a layered decomposition~\cite{srikanthan2023augmented}, we apply the ADMM algorithm to~\eqref{prob:library-ocp}, yielding the following iterative updates 
\begin{subequations}\label{prob:ocp_admm}
    \begin{align}
        \boldsymbol{\bar{z}}^{k+1} &\coloneqq \argmin\limits_{\boldsymbol{\bar{z}}} \boldsymbol{J}(\boldsymbol{\bar{z}};\xi_g) + \frac{\rho}{2} \left \| \boldsymbol{z}^k - \boldsymbol{\bar{z}} + \boldsymbol{v}^k \right \|_2^2 \nonumber \\
        % \begin{bmatrix}
        %     \boldsymbol{x}^k - \boldsymbol{r_p} + \boldsymbol{v_{r,p}}^k \\
        %       \boldsymbol{u}^k - \boldsymbol{a_p} + \boldsymbol{v_{a,p}}^k 
        %  \end{bmatrix} \right\Vert_2^2 \nonumber \\
        \text{s.t. } & \bar{\psi}(\boldsymbol{\bar{z}}; w_p) = 0, \label{eq:trajectory-gen} \\
        \boldsymbol{z}^{k+1} &\coloneqq \argmin_{\boldsymbol{z}} \ \frac{\rho}{2} \| \boldsymbol{z} - \boldsymbol{\bar{z}}^{k+1} + \boldsymbol{v}^k \| \nonumber \\
        % \left\Vert \begin{bmatrix}
        %     \boldsymbol{x_p} - \boldsymbol{r_p}^{k+1} + \boldsymbol{v_{r,p}}^k \\
        %       \boldsymbol{u_p} - \boldsymbol{a_p}^{k+1} + \boldsymbol{v_{a,p}}^k
        %  \end{bmatrix} \right \Vert_2^2 \nonumber \\
        \text{s.t. } & \psi(\boldsymbol{z}, \xi) = 0 \label{eq:fb-control} \\
        % & \quad \text{s.t. } x_{t+1} = f(x_t, u_t), \ t=0, \dots, N-1  \nonumber\\
        % & \quad \quad \ \, x_0 = \xi \\
        \boldsymbol{v}^{k+1} &\coloneqq \boldsymbol{v}^k + \boldsymbol{z}^{k+1} - \boldsymbol{\bar{z}}^{k+1} \label{eq:dual-update},
        % \boldsymbol{v_{r,p}}^{k+1} &\coloneqq \boldsymbol{v_{r,p}}^k + \boldsymbol{x_p}^{k+1} - \boldsymbol{r_p}^{k+1} \nonumber \\
        % \boldsymbol{v_{a,p}}^{k+1} &\coloneqq \boldsymbol{v_{a,p}}^k + \boldsymbol{u_p}^{k+1} - \boldsymbol{a_p}^{k+1} \label{eq:dual-update},
\end{align}
\end{subequations}
where $\boldsymbol{z, \bar{z}}$ are primal variables, $\boldsymbol{v}$ is a scaled dual variable and $\rho$ is a tuning parameter to improve convergence of the ADMM algorithm. Moreover~\eqref{eq:trajectory-gen} is a time separable feasibility problem  without dynamics constraints that can benefit from parallelization, while~\eqref{eq:fb-control} is an unconstrained OCP with nonlinear dynamics and a quadratic objective function which can be solved via sequential linearization-based techniques, such as iLQR. Finally, the dual updates in~\eqref{eq:dual-update} ensure consistency so as to guarantee both constraint satisfaction and dynamic feasibility at convergence. We note here that one could choose any constrained optimization method to solve~\eqref{prob:library-ocp}, however, using the proposed ADMM-based decomposition facilitates computing feedback gain matrices, as discussed below. 

If $\boldsymbol{J}$ is convex, the only nonconvex part of the problem is the \emph{unconstrained} nonlinear dynamics found in the update step~\eqref{eq:fb-control}. By isolating the nonconvexity of the problem to this update step, we can leverage iLQR~\cite{todorov2005generalized} to rapidly converge to a locally optimal solution under fairly benign assumptions~\cite{liao1991convergence}. In what follows, we show how we solve~\eqref{eq:fb-control} using iLQR, resulting in local convergence to an optimal feedback controller that tracks the reference trajectory $\boldsymbol{\bar{z}}$ from~\eqref{eq:trajectory-gen}. 
% To guarantee convergence of iLQR, we warmstart the~\eqref{eq:fb-control} from dynamically feasible $\boldsymbol{z}$ obtained from the previous ADMM iteration.

\subsubsection{Feedback controller from ADMM iterates}
\label{sec: nom fd controller}
For any ADMM iteration $k+1$, let $\boldsymbol{d}^k = -(\boldsymbol{z}^k - \boldsymbol{\bar{z}}^{k+1} + \boldsymbol{v}^k)$. By doing a change of variable from $\boldsymbol{x, u}$ to $\boldsymbol{\delta x} = \boldsymbol{x} - \boldsymbol{x}^k$ and $\boldsymbol{\delta u} = \boldsymbol{u} - \boldsymbol{u}^k$, and setting $\boldsymbol{\delta z} = (\boldsymbol{\delta x^\top, \delta u^\top})^\top$, the feedback control problem in~\eqref{eq:fb-control} is approximately solved via iLQR:
% \begin{equation}\label{eq:nonlin-track-layer}
%     \boldsymbol{\delta z}^{\ell+1} \coloneqq \argmin_{\boldsymbol{\delta z}}\ \frac{\rho}{2}\| \boldsymbol{\delta z} - \boldsymbol{d}^{\ell} \|_2^2 \nonumber \quad \text{s.t. } \delta z_{x,i+1} = \begin{bmatrix}
%             A_i^{\ell} & B_i^{\ell} \end{bmatrix}
%             \delta z_i
% \end{equation}
\begin{align}
    \boldsymbol{\delta z}^{\ell+1} \coloneqq &\argmin_{\boldsymbol{\delta z}}\ \frac{\rho}{2}\| \boldsymbol{\delta z} - \boldsymbol{d}^{\ell} \|_2^2 \nonumber \\
        &\text{s.t. } \delta z_{x,i+1} = \begin{bmatrix}
            A_i^{\ell} & B_i^{\ell} \end{bmatrix}
            \delta z_i \label{eq:nonlin-track-layer} 
        % \frac{\partial}{\partial \boldsymbol{z}} \psi(\boldsymbol{z};\xi) |_{\boldsymbol{z} = \boldsymbol{z}^{k+\ell}} = 0 
        % \delta x_{i+1, p} &= A_{i, p}^{\ell} \delta x_{i, p} + B_{i, p}^{\ell} \delta u_{i, p}, \ \forall i \geq 0,  \label{eq:nonlin-track-layer}
        % & \quad x_{0, p} = \xi
        % \mathbf{v}^{k+1} &\coloneqq \mathbf{v}^k + \mathbf{x}^{k+1} - \mathbf{r}^{k+1}. \label{eq:nonlin-dual-update}
\end{align}
where $\ell$ is iLQR iteration counter and the constraint in~\eqref{eq:nonlin-track-layer} is from linearization of the dynamics constraints $f_d$ with $\begin{bmatrix}
    A_i^{\ell} & B_i^{\ell}
\end{bmatrix} = \frac{\partial f_d(z)} {\partial z}|_{z=z^{k+\ell}}$. Solving~\eqref{eq:nonlin-track-layer} using dynamic programming results yields time-varying feedback gain matrices $\calK_{i, p}^\star$~\cite{todorov2005generalized}. 
Once the ADMM algorithm has converged, for the $p$th nominal controller at any discrete-time index $i$ we have
\begin{equation}\label{eq:ctrl-params}
    \mu_{i, p}^\star, \quad \calK_{i, p}^\star, \quad x_{i, p}^\star
\end{equation} 
the nominal input, the feedback gain matrices, and the resulting state vector respectively. We report the time taken for convergence of the algorithm with different sampling times ($T_s$) and trajectory horizons ($T$) in Table~\ref{tab:admm}. We next illustrate how the feedback gain matrices from each nominal controller $\calK_{i, p}^\star$ play a role in stabilizing the system online whenever the MCBF safety filter modifies the nominal inputs.

% Since this is a standard derivation from prior work~\cite{todorov2005generalized}, we omit it in our presentation.
% The linearization at $(x_{i, p}^{k+\ell}, u_{i, p}^{k+\ell})$ is such that $A_{i, p}^{\ell} = \frac{\partial f_d(x, u)} {\partial x}|_{x=x_{i, p}^{k + \ell}, u=u_{i, p}^{k + \ell}},\ B_{i, p} = \frac{\partial f_d(x, u)}{\partial u}|_{x=x_{i, p}^{k + \ell}, u=u_{i, p}^{k + \ell}}$.
% We also note that the cost terms appearing in~\eqref{eq:nonlin-track-layer} only depend on $\boldsymbol{\delta z}$ since $\boldsymbol{d}^{\ell}$ is a parameter and not an optimization variable. Hence, the feedback control layer is a standard iLQR whose initial parameters are ``warm starts" obtained from previous solutions of ADMM. We solve problem~\eqref{eq:nonlin-track-layer} until iLQR converges to a locally optimal solution. 

% Say, at ADMM iteration $k+1$ iLQR converges after $M$ iterations, then the resulting closed-loop feedback law is given by 
% \begin{equation}\label{eq:closed-loop-fb-law}
%     \mu_{i, p}^{k+1} := u_{ff, i}^{k+M} - K_{i, p}^{M} \delta x_{i, p}^{M}.
% \end{equation}
% where $\mu_{i, p} \in \R^m$ is the feedback controller obtained for nominal controller $p$ mapping to a control input at each time step $i$. We highlight here that  our application of the ADMM algorithm results in a 2DOF design pattern with a feedforward and feedback term. 


% Although we do not guarantee convergence of ADMM, we observe that using slack variables for waypoint constraints in the optimization significantly improves convergence. In addition, we choose a cost function for problem~\eqref{eq:trajectory-gen} that encourages smooth trajectories for a given dynamical system without incurring any additional computational costs. 
% In the next section, we show how the feedback gain matrices from each nominal controller $\calK_{i, p}^\star$ play a role in stabilizing the system online whenever the MCBF safety filter modifies the nominal inputs. 

% For more details on the derivation, please refer to the Appendix. We highlight here that  our application of the ADMM algorithm results in a 2DOF design pattern with a feedforward and feedback term. Once the ADMM algorithm has converged, we use $\mu_p^\star(\cdot)$ to denote the nominal input from controller $p$ and the feedback gain matrix as $\calK_{p}^\star(\cdot)$. In the next section, we show how the feedback gain matrices from each nominal controller $\calK_{p}^\star(\cdot)$ play a role in stabilizing the system online whenever the CBF safety filter modifies the nominal inputs. 

% Therefore, In the following section, we describe how we select trajectories online and achieve guaranteed obstacle avoidance.
% Next, we state the feedback control law with 2DOF structure when the ADMM algorithm~\eqref{prob:ocp_admm} has converged. 
% When applying the controller in conjunction with CBF, we first run the layered control system to convergence to obtain the converged nominal controller. We modify the feed-forward term in the nominal controller using CBF and the feedback term is used as a smoothing filter. 

% To use the smoothing filter, use converged $A_t^*, B_t^*$ to rollout the dynamics for $\delta u = u_{mod} - u_{nom}$ and $\delta x = x_{obs} - x_{des}$ to get $\delta x_{t+1}$ and then apply $K_t$ to bring the system to the new state.

% We denote the state trajectory by $\mathbf{x}:=(x_{0|t},x_{1|t},\dots,x_{T|t}) \in \mathbb{R}^{n \times (T+1)}$, the control input trajectory by $\mathbf{u}:=(u_0,u_{1},\dots,u_{N-1}) \in \mathbb{R}^{m \times T}$, 
%  and $\mathbf{c}(\mathbf{x, u}):= \sum_{t=0}^{T-1} c_t(x_{t},u_{t})$,  the stage cost over trajectories. We define constraints at time $i$ as 
% \begin{align}
%     \psi_i(x_{i|t}, u_{i|t})  &=  \begin{cases}
%         0 \quad &\text{if $(x_{i|t}, u_{i|t}) \in \mathcal{X}\times \mathcal{U},$}  \\
%         \infty \quad &\text{otherwise}
%     \end{cases}, \qquad \forall 0\leq i<T\\
%     \psi_T(x_{T|t}, u_{T|t}) &=  \begin{cases}
%         0 \quad &\text{if $x_{T|t} \in \mathcal{X}_f$}  \\
%         \infty \quad &\text{otherwise}
%     \end{cases}  
% \end{align} and $\psi^T(\vec z) = \sum_{t=0}^{T} \psi_t(x_{i|t}, u_{i|t})$, where $\mathcal{X}_f$ denotes a terminal constraint set to be defined later. We also define dynamic constraints at time $i$ as 
% \begin{align}
%     \Bar{\psi}_i(x_{i+1|t})  &=  \begin{cases}
%         0 \quad &\text{if $x_{i+1|t} = Ax_{i|t} + Bu_{i|t} ,$}  \\
%         \infty \quad &\text{otherwise}
%     \end{cases}, \qquad \forall 0\leq i<T\\
%     \Bar{\psi}_0(x{0|t}) &=  \begin{cases}
%         0 \quad &\text{if $x_{0|t} = \xi$}  \\
%         \infty \quad &\text{otherwise}
%     \end{cases}  
% \end{align}

% Given a discrete-time nonlinear system of the form
% \begin{equation}\label{eq:ct-dynamics}
% x(t+1) = f(x(t), u(t))
% \end{equation}
% where $f$ is derived from the mechanical dissipativity or Euler-Lagrange equations of the system, we want to design a controller that satisfies input constraints; while ensuring that the resulting states satisfy static and dynamic obstacle avoidance constraints with real-time performance guarantees. Such constraints are typically specified as Solving an optimal control problem with state and input constraints over long horizons and running them in open loop will work poorly since 

% To achieve this, we 

% To design a controller, consider a discrete-time dynamical system obtained by RK45 discretization of $f$ as follows
% \begin{equation}
%     x(t+1) = f_d(x(t), u(t))
% \end{equation}
% Static obstacle constraints and actuator limits could be incorporated as state and input constraints if we have prior knowledge of obstacle locations. Consider a discrete-time finite-horizon optimal control problem (OCP) with initial $x(0) = \xi$ and terminal condition $x(N) = \xi_g$ as follows:
% \begin{equation}\label{prob:ocp}
% \begin{array}{rl}
%      \mathrm{minimize} & \sum_{t=0}^{N-1} q(x(t)) + \Vert u(t) \Vert_R^2 \\
%      % \text{subject to} &  x(t+k+1) = Ax(t+k) + Bu(t+k), \\
%      \text{subject to} &  x(t+1) = f_d(x(t), u(t)), \\
%      & x(t) \in \mathcal{X},\ u(t)) \in \U,\ \forall t\geq 0 \\
%      & x(N) = \xi_g \\
%      & x(0) = \xi
% \end{array}
% \end{equation}
% where $x(k) \in \R^n$, $u(k) \in \R^m$ are state and input vectors, $\mathcal{X} \subseteq \R^n, \mathcal{U} \subseteq \R^m$ are state and input constraint sets respectively, and $\xi, \xi_g$ are initial and terminal states respectively, and $R \in \R^{m\times m}$ is an input weight matrix. 

% In the next sub-section, we contextualize our problem for designing a controller for a differential drive robot using a reduced-order model and layout the challenges that arise from such a methodology. Following this, we propose our framework for a systematic synthesis of a layered control architecture to navigate a differential-drive robot under different model assumptions showing its benefit over the current state-of-the-art. allows the CBF to loosen constraints  robustify collision-free path-planning for differential drive robots. 

% Now, we want to study the closed loop behavior when a sub-optimal policy constructed by a splitting method approximately solves~\eqref{eq:linear_ocp}. To construct our sub-optimal policy, we first introduce  auxiliary variables $\mathbf{r_{x}} := \mathbf{x},\; \mathbf{r_u}:=\mathbf{u}$  and  denote $\mathbf{r_{z}}:=[\mathbf{r_x}^\top,\mathbf{r_u}^\top]^\top$. Consider, then, the following optimization problem and some initial $\mathbf r_z^0 \in\mathbb{R}^{s}, \; \mathbf z^0 \in \mathbb{R}^{s}$ and $\mathbf v^0 \in \mathbb{R}^{s} $ with $s:=m N + n (N+1)$, to be solved in a receding horizon fashion at each time $t$ after $x(t)$ has been measured
% \begin{subequations}\label{eq:linear_ocp_admm}
%     \begin{align}
%         (\mathbf r_z^{k+1}) &\coloneqq \argmin_{\mathbf{r_z}}  \frac{1}{2}\mathcal{C}^T(\mathbf r_z) + \psi^T(\mathbf{r_z}) + \frac{\rho}{2} \Vert \mathbf{r_z} -\mathbf{z}^k  + \mathbf {v}^k \Vert_2^2 
%         %& \quad \text{s.t. }\  r_{x,N} = \xi_g %\ak{?r_{x,0} = x_0?}, \
%         \label{eq:linear-ref-layer} \\
%         \left(\mathbf z^{k+1}\right) &\coloneqq \argmin_{\mathbf {z}}  \frac{1}{2}\mathcal{C}^T(\mathbf {z}) + \Bar{\psi}^T(\mathbf z) + \frac{\rho}{2} \left\Vert
%             \mathbf r_z^{k+1} - \mathbf {z} + \mathbf v^k \right \Vert_2^2 \label{eq:linear-control-update}\\
%         % & \quad \text{s.t. } x_{i+1|t} =f_0(x_t) + g(x_t,u_t), \ i=0, \dots, T-1  \nonumber\\
%         % &\quad  \quad  z_i = \left[x_t^\top,~u_t^\top\right]^\top  \ i=0, \dots, T-1 \nonumber,\\
%         % & \quad \ \, x_{0|t} = x_t \nonumber, \\
%         \mathbf {v}^{k+1} &\coloneqq \mathbf {v}^k +  \mathbf r_z^{k+1} - \mathbf {z}^{k+1},
%         \label{eq:linear-dual-update}
% \end{align}
% \end{subequations}
% where we denote the combined state, input and dual variables as $\mathbf \varphi^k := (\varphi_0^k, \cdots, \varphi_T^k) \in \mathbb{R}^{m\times N + 2n\times (N+1)}$ with $\varphi_i^k:=\begin{bmatrix}
%     z_i^k \\ v_i^k
% \end{bmatrix} \in \mathbb{R}^{2n+m}$ and $z_i = \left[x_t^\top,~u_t^\top\right]^\top$. If~\eqref{eq:linear_ocp_admm} is run until convergence, then  it corresponds to the optimal MPC policy~\eqref{eq:rhc-law}. Moreover, with an appropriately defined prediction horizon $T$, it is stabilizing the closed-loop system. In particular, given an initial state $\xi\in \mathbb{R}^n$ as a parameter, we denote the converged solution of \eqref{eq:linear_ocp_admm} by $(\mathbf r_z^\star(\xi), \mathbf z^\star(\xi), \mathbf v^\star(\xi))$, mapping the parameter $\xi$ to the optimal primal and dual variables. The closed-loop system under this optimal MPC policy is then given by
% \begin{equation}\label{eq:optimal_closed_loop}
%     x^\star(t+1) = Ax^\star(t) + B\Xi \mathbf \varphi^\star(x_t^\star):= \bar{f}(x_t^\star),
% \end{equation}
% where $\Xi$ is an appropriately defined selector matrix, that selects the first control input $u^\star_{0|t}$ at each time step $t$. We denote by $\Bar{f}(\cdot)$ the closed-loop dynamics under the optimal MPC policy $\varphi^\star(\cdot)$. 

% Here, we show how to derive a two-layer and three-layer control architecture for designing a nominal controller for $f_d$. As a first step, we introduce redundant reference variables $r(t), a(t),\ \forall t \geq 0$ constrained to satisfy $r(t) = x(t), a(t) = u(t),\ \forall t \geq 0$ to the optimal control problem in~\eqref{prob:ocp} as shown below: 
% \begin{equation}\label{prob:redundant-ref-var}
% \begin{array}{rl}
%      \mathrm{minimize} & \sum_{t=0}^{N-1} q(r(t)) + \Vert u(t) \Vert_R^2 \\
%      % \text{subject to} &  x(t+k+1) = Ax(t+k) + Bu(t+k), \\
%      \text{subject to} &  x(t+1) = f_d(x(t), u(t)), \\
%      & r(t) \in \mathcal{X},\ u(t)) \in \U,\ \forall t\geq 0 \\
%      & r(0) = \pi(\xi), \ r(N) = \xi_g, \\
%      & \mathbf{r} = \pi(\mathbf{x}),\ \mathbf{a} = \mathbf{u} 
% \end{array}
% \end{equation}
% where $\mathbf{r} = (r(0),r(1),\dots,r({N}))$ and $\mathbf{a} = (a(0),a(1),\dots,a({N-1}))$ and the constraint sets $\mathcal{X, U}$ are polytopes. We note here that the reference variables are suitably chosen to replace the cost functions and constraints, however, the dynamics equations are left to be 
% % We now show how solving~\eqref{eq:redundant-ref-var} using ADMM naturally yields solutions with a 2DOF layered control architecture.

%state the framework of 2DOF  resulting from applying ADMM to the optimization problem in~\eqref{eq:redundant-ref-var} and discuss the implications of each step of the ADMM updates in detail.

% \subsection{Reduced-order Two-layer Control Architecture (r2-LCA)}

% Instead of introducing redundant variables that are ``dynamics-free", we introduce variables $\mathbf{s,\mu}$ which follow a reduced-order dynamics model $\Bar{f}$. Introducing the redundant variable and dynamics to problem~\eqref{prob:ocp}, we have
% \begin{equation}\label{prob:reduced-ocp}
% \begin{array}{rl}
%      \mathrm{minimize} & \sum_{t=0}^{N-1} q(s(t), \mu(t)) + \Vert u(t) \Vert_R^2 \\
%      \text{subject to} &  s(t+1) = \Bar{f}(s(t), \mu(t)), \\
%      & s(t) \in \mathcal{X}_s,\ \mu(t)) \in \mathcal{X}_s^{\dagger},\ \forall t\geq 0 \\
%      & s(0) = \pi(\xi), \mu(0) = (I-\pi)(\xi), \\
%      & s(N) = \pi(\xi_g),\ \mu(N) = (I-\pi)(\xi_g), \\
%      &  x(t+1) = f_d(x(t), u(t)), \\
%      & \mathbf{s} = \pi(\mathbf{x}),\ \mathbf{\mu} = (I-\pi)(\mathbf{x}) 
%      % \text{subject to} &  x(t+k+1) = Ax(t+k) + Bu(t+k), \\
% \end{array}
% \end{equation}


% Applying the layered decomposition proposed from~\cite{srikanthan2023augmented} to~\eqref{prob:reduced-ocp}, we get the following architecture
% \begin{subequations}\label{prob:reduced-admm}
%     \begin{align}
%         \mathbf{(s^{k+1}, \mu^{k+1})} &\coloneqq \argmin_{\mathbf{s, \mu}} \ q(\mathbf{s, \mu}) +  \frac{\rho}{2} \left\Vert \begin{bmatrix}
%             \pi(\mathbf{x}^k) - \mathbf{s} + \mathbf{v_x}^k \\
%               (I-\pi)\mathbf{x}^k - \mathbf{\mu} + \mathbf{v_u}^k 
%          \end{bmatrix} \right\Vert_2^2 \nonumber \\
%         \text{s.t. } & \quad s(t+1) = \Bar{f}(s(t), \mu(t)), \nonumber \\
%         & \quad s(t) \in \mathcal{X}_s,\ \mu(t) \in \mathcal{X}_s^{\dagger},\ \forall t \geq 0, \nonumber \\
%         & \quad s(0) = \pi(\xi), \mu(0) = (I-\pi)(\xi), \nonumber \\
%      & \quad s(N) = \pi(\xi_g),\ \mu(N) = (I-\pi)(\xi_g),\label{eq:red-trajectory-gen} \\
%         \left(\mathbf{x}^{k+1}, \mathbf{u}^{k+1}\right) &\coloneqq \argmin_{\mathbf{x, u}} \ \frac{\rho}{2} \left\Vert \begin{bmatrix}
%             \pi(\mathbf x) - \mathbf s^{k+1} + \mathbf v_{x}^k \\
%               (I-\pi)\mathbf x - \mathbf \mu^{k+1} + \mathbf v_{u}^k
%          \end{bmatrix} \right \Vert_2^2 + \mathbf u^T R \mathbf u \nonumber \\
%         \text{s.t. } & \quad x(t+1) = f_d(x(t), u(t)),\ x(0) = \xi \nonumber \\
%         & \quad u(t) \in \U, \ \forall t \geq 0 \\
%         % & \quad \text{s.t. } x_{t+1} = f(x_t, u_t), \ t=0, \dots, N-1  \nonumber\\
%         % & \quad \quad \ \, x_0 = \xi \\
%         \mathbf{v_x}^{k+1} &\coloneqq \mathbf{v_x}^k + \pi(\mathbf{x}^{k+1}) - \mathbf{s}^{k+1} \nonumber \\
%         \mathbf{v_u}^{k+1} &\coloneqq \mathbf{v_u}^k + (I-\pi)\mathbf{x}^{k+1} - \mathbf{\mu}^{k+1}. 
% \end{align}
% \end{subequations}
% where $\pi$ is a projection matrix that projects the states to reduced-order states like x,y position and heading angle ($x_1, x_2, \theta$) and inputs like linear and angular velocity $(v, \omega)$.

%Here we describe how the ADMM algorithm, as applied to solving OCP~\eqref{eq:redundant-ref-var}, naturally yields a layered control architecture.  In particular, ADMM iterates between updating the reference trajectory $\mathbf r$, the state and control trajectories $(\mathbf x, \mathbf u)$, and the Lagrange multipliers $\mathbf v$ that ensure consistency between state $\mathbf x$ and reference $\mathbf r$ trajectories.

% We describe how the ADMM iterate updates~\eqref{eq:admm_ocp} can be interpreted as a layered control architecture:
% \begin{enumerate}[label=\alph*)]
%     \item \textbf{Trajectory generation layer~\eqref{eq:ref-layer}:} The $\mathbf r$-update step~\eqref{eq:ref-layer} is naturally interpreted as a trajectory generation layer, wherein an updated reference trajectory $\mathbf{r}$ is obtained by optimizing the the utility cost $C_x(\mathbf r)$ subject to state constraints $\mathbf r \in \mathcal R^N$.  While the reference trajectory is not explicitly constrained to be dynamically feasible a trust-region-like penalty $\frac{\rho}{2}\Vert \mathbf{x}^k - \mathbf{r} + \mathbf{v}^k \Vert_2^2$ arising from the augmented Lagrangian regularizes the reference trajectory to be approximately consistent with the current (dynamically feasible) state trajectory $\mathbf x^k$.
%     \item \textbf{Feedback control layer~\eqref{eq:track-layer}:} We immediately recognize the $(\mathbf x, \mathbf u)$-update step~\eqref{eq:track-layer} as a reference tracking optimal control problem, with reference given by $\mathbf r^{k+1} - \mathbf v^k$.  Depending on the problem setting, exact or approximate optimal feedback controllers can be obtained to this update step.
%     \item \textbf{Dual update~\eqref{eq:dual-update}:} Finally, the dual variables $\mathbf v$ are updated according to equation~\eqref{eq:dual-update}.  We notice that the dual variable $\mathbf v$ can be seen as a protocol between the trajectory generation and feedback control layers that ensure that the planned reference trajectories converge to dynamically feasible behaviors (and vice versa).
% \end{enumerate}

% \subsection{Three-layer Control Architecture (3-LCA)}

% \anusha{Is this even needed?} Here we describe how to obtain a three layered architecture such that the middle layer introduces a reduced order dynamics model $\Bar{f}$ for the discrete-time nonlinear system $f_d$. We introduce redundant variables $\mathbf{s, v, r, a}$ such that $\mathbf{s, v}$ are reduced order states and inputs respectively and $\mathbf{r, a}$ will introduce a layer that has no dynamics. TODO

% \begin{subequations}
%     \begin{align}
%         \mathbf{(r^{k+1}, a^{k+1})} &\coloneqq \argmin_{\mathbf{r, a}} \frac{\rho}{2} \left\Vert \begin{bmatrix}
%             \pi(\mathbf{x}^k) - \mathbf{r} + \mathbf{v_r}^k \\
%               \mathbf{u}^k - \mathbf{a} + \mathbf{v_a}^k 
%          \end{bmatrix} \right\Vert_2^2 \nonumber \\
%         &\quad \text{s.t. } a(t) \in \mathcal{U},\ \forall t \geq 0 \label{eq:trajectory-gen} \\
%         \mathbf{(r^{k+1}, a^{k+1})} &\coloneqq \argmin_{\mathbf{s, v}} \ q(\mathbf{s, v}) +  \frac{\rho}{2} \left\Vert \begin{bmatrix}
%             \mathbf{x}^k - \mathbf{(s, v)} + \mathbf{\mu}^k 
%          \end{bmatrix} \right\Vert_2^2 \nonumber \\
%         &\quad \text{s.t. } s(t) \in \mathcal{X}_s,\ v(t) \in \mathcal{X}_s^{\dagger},\ \forall t \geq 0 \label{eq:trajectory-gen} \\
%         \left(\mathbf{x}^{k+1}, \mathbf{u}^{k+1}\right) &\coloneqq \argmin_{\mathbf{x, u}} \ \frac{\rho}{2} \left\Vert \begin{bmatrix}
%             \mathbf x - \mathbf r^{k+1} + \mathbf v_{r}^k \\
%               \mathbf u - \mathbf a^{k+1} + \mathbf v_{a}^k
%          \end{bmatrix} \right \Vert_2^2 + \mathbf u^T R \mathbf u \nonumber \\
%         & \text{s.t. } x(t+1) = f_d(x(t), u(t)),\ x(0) = \xi\\
%         % & \quad \text{s.t. } x_{t+1} = f(x_t, u_t), \ t=0, \dots, N-1  \nonumber\\
%         % & \quad \quad \ \, x_0 = \xi \\
%         \mathbf{v_r}^{k+1} &\coloneqq \mathbf{v_r}^k + \mathbf{x}^{k+1} - \mathbf{r}^{k+1} \nonumber \\
%         \mathbf{v_a}^{k+1} &\coloneqq \mathbf{v_a}^k + \mathbf{u}^{k+1} - \mathbf{a}^{k+1}. 
% \end{align}
% \end{subequations}


==> tex/4b-CBFs.tex <==
% \subsection{Online Execution}
\subsection{Online Safe Reactive Control}

% In the previous subsection, we discussed the details of offline path library generation by using a fixed set of waypoints to sufficiently cover the exploration space of the robot as shown in Figure~\ref{fig:intro-block-diag}. 
% The offline nominal controller library generation gives us instantaneous access to nominal controllers for the entire horizon $T$ without having to do any re-computation online. Further, 
In this section, we first describe the MCBF controller we solve online using the selected nominal inputs and provide details of our proposed architecture in the green block of Figure~\ref{fig:intro-block-diag}.

\begin{figure}[t]
    \centering
    % \subfloat[\label{2a}]{
    %     \centering  
    %     \includegraphics[width=0.45\columnwidth, height=1.2in]{img/front_and_back_nom_traj_new.png}
    %     \label{fig:multi-path-admm}
    % } 
    % % \hfill
    % \subfloat[\label{2b}]{
    %     \centering
    %     \includegraphics[width=0.45\columnwidth, height=1.2in]{img/exploration space.png}
    %     \label{fig:hospital}
    % }
    % \centering
    \begin{subfigure}{0.49\linewidth}
         \includegraphics[width=\textwidth]{img/front_and_back_nom_traj_new.png}
    % \vspace{-5pt}
    \caption{\label{fig:multi-path-admm}}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
         \includegraphics[width=\textwidth]{img/exploration_space.png}
     \caption{\label{fig:hospital}}
    \end{subfigure}
    \caption{\label{fig:online-execution}In~\ref{fig:multi-path-admm}, we show the feasible trajectories from our path library in green visualizing the computed offline solutions for the initially unknown environment in~\ref{fig:hospital}. The pink dots indicate the feasible next states to choose from. The nearby detected obstacle boundaries are visualized as blue point clouds. }   
    \vspace{-20pt}
\end{figure}
% At each time step $t$, we use nearest neighbor search to choose the closest trajectory to guide the robot towards the goal with feasible nominal inputs while still maintaining safety through a MCBF safety filter.

\subsubsection{Reactive Control with MCBF} While our proposed LCA could use any reactive strategy, to generate safe inputs that ensure no local minima we use the modulation based on-Manifold Modulated CBF-QP (MCBF-QP) \cite{xue2024nominima}. Control inputs synthesized by CBF-QPs inevitably result in saddle points even for fully-actuated robots (see ~\cite[Thm. 5.3]{xue2024nominima}). To eliminate the saddle points of CBF-QP solvers and their variants, MCBF-QP modulates the dynamics and projects components onto the tangent planes of the obstacle boundary functions, introducing tangential velocities. This is achieved by introducing an additional constraint on the standard CBF-QP formulations as in~\eqref{eq:mod-phi-cbf constraint affine}. The MCBF-QP is presented below:
% \begin{equation}
%     \phi(x,t)^\top f(x)+\phi(x,t)^\top g(x)(u -u_\text{nom})\geq \gamma. \label{eq:mod-phi-cbf constraint affine}
% \end{equation}
\begin{gather}\label{eq:mod-phi-cbf affine} 
\nonumber u_{\text{mcbf}} = \argmin_{u \in \mathbb{R}^p}\;(u-u_\text{nom})^\top(u-u_\text{nom})\\
L_fh(x,x_o) + L_gh(x,x_o)u + \nabla_{x_o}h(x,x_o)\dot{x}_o\geq -\alpha (h(x,x_o))\\
\phi(x,x_o)^\top f(x)+\phi(x,x_o)^\top g(x)u \geq \gamma, \label{eq:mod-phi-cbf constraint affine}
\end{gather}
where $L_f$ and $L_g$ are the Lie derivatives of $h(x, x_o)$. Here, $\gamma$ is the user's choice of a strictly positive real number, and the tangent direction $\phi(x, x_o)$ can be derived using various obstacle exit strategies, such as hessian or geometric approximation. See \cite{xue2024nominima} and \cite{onManifoldMod} for implementation details.
% The resulting MCBF filter eliminates local minima for unsafe sets of all geometric types, including non-star-shaped obstacles, as shown in \cite{xue2024nominima}. 

\subsubsection{Online Path Selector} To achieve obstacle avoidance in real-time and ensure task completion, we initialize the path at $t=0$ using the center-line connecting initial state to the goal. For $t>0$, we first run a nearest neighbor search algorithm to decide which path to track:
\begin{equation}
    p^\star(t+1) = \argmin_p \| \{x_{i, p}^\star\}_{p=0}^N - x_{pred}(t+1) \|,
\end{equation}
where $x_{pred}(t+1) = f_d(x(t), u_{mcbf}(t))$ with $u_{mcbf}(t)$ as the optimized input from solving MBCF-QP~\eqref{eq:mod-phi-cbf affine}.
% ~\eqref{eq:mod-phi-cbf affine}. 
Ties are broken by selecting the one closer to the center-line connecting the initial state to the goal. Once we obtain $p^\star(\cdot)$, we construct the nominal input with a feedback term as 
\begin{equation}\label{eq:nominal-inp}
    u_{nom}(t) = \mu_{i, p^\star}^\star + \calK_{i, p^\star}^\star(x_{i, p^\star}^\star - x(t)).
\end{equation}
%Next, we apply the MCBF filter % solving~\eqref{eq:mod-phi-cbf affine} 
%to ensure obstacle avoidance, and command the robot. 
The feedback control law in~\eqref{eq:nominal-inp} has a feedforward term $\mu_{i, p^\star}$ that drives the robot toward the goal in the absence of obstacles. When the robot is near an obstacle, the feedback term $\calK_{i, p^\star}^\star$ is a proportional compensation for deviations from the nearest $x_{i, p^\star}^\star$ resulting in a smooth transition between paths. We emphasize that these feedback gain matrices $\calK_{i, p^\star}^\star$ are derived from~\eqref{prob:ocp_admm}, not tuned manually. When no obstacles are present, $u_{mcbf} \approx u_{nom}$, while in obstacle situations, $\calK_{i,p^\star}$ compensates for the deviations. Our online execution runs at 100 Hz, solving in under 0.01 seconds on average.

% The key insight is in using time-varying feedback gain matrices $\calK_{i, p^\star}^\star$ to construct a ``proportional term'' to stabilize the system when the nominal input~\eqref{eq:nominal-inp} is modified. 


% While our proposed LCA could use any reactive strategy, to generate safe inputs that guarantee no local minima we use the modulation based on-Manifold CBF-QP (MCBF-QP) \cite{xue2024nominima}. To overcome the saddle points of CBF-QP solvers and their variants, MCBF-QP modulates the dynamics and projects components onto the tangent planes of the obstacle boundary functions, introducing velocities that eliminate saddle points. This is achieved by introducing an additional constraint on the standard CBF-QP formulations defined as \eqref{eq:mod-phi-cbf constraint affine}, 
% \begin{equation}
%     \phi(x,t)^\top f(x)+\phi(x,t)^\top g(x)(u -u_\text{nom})\geq \gamma. \label{eq:mod-phi-cbf constraint affine}
% \end{equation}
% Here, $\gamma$ is the user's choice of a strictly positive real number, and the tangent direction $\phi(x)$ can be derived using various obstacle exit strategies, such as hessian or geometric approximation. See \cite{xue2024nominima} and \cite{onManifoldMod} for implementation details. 
% projected onto the tangent hyperplane $H(x,t)$ using $\phi(x,t)$. $\phi(x,t)$ can be solved using geometric approximation methods, the details of which can be found in \cite{onManifoldMod}.
% The parameter $\gamma$ is a user-defined positive real number, i.e. $\gamma \in \mathbb{R}^+$ \cite{MCBF}.
% \begin{gather}\label{eq:mod-phi-cbf affine} 
% \nonumber u_{\text{mcbf}} = \argmin_{u \in \mathbb{R}^m}(u-u_\text{nom})^T(u-u_\text{nom})\\
% \Dot{h}(t, x, u) =L_fh(t, x) + L_gh(t, x)u + \frac{\partial h(t, x)}{\partial t}\geq -\alpha (h(t, x))\\
% \phi(x,t)^Tf(x)+\phi(x,t)^Tg(x)(u -u_\text{nom})\geq \gamma. \label{eq:mod-phi-cbf constraint affine}
% \end{gather}

% The resulting MCBF filter eliminates local minima for unsafe sets of all geometric types, including non-star-shaped obstacles, as proven in \cite{xue2024nominima}. %Validations of MCBF in avoiding concave obstacles can be found in~\cite{xue2024nominima}. 
% the stuck in local minima induced by the selected safety filter. Therefore, here we argue that for control affine systems in general, the local-minimum free safety filter of Mod-based on-Manifold CBF (MCBF) is the superior choice.  


% What this means is that $u_{mcbf} = u_{nom}$ when there are no obstacles in the robot's path. Whenever, there are obstacles, $u_{nom}(t+1)$ uses the feedback gain matrix $\calK_{i, q}$ to guide the robot towards desired next states. Having several options in our library enables us to transition from one path to the next seamlessly. Our online execution scheme solves in under 0.01 seconds on average and can run at 100 Hz. 

% After the robot moves, the robot's state becomes $x(t+1)$. 
% The index $i$ is incremented every $t+T_s$ seconds, provided there are no system delays. Instead of measuring delays directly, we quantify the robot's progress to $x_{i, q}^\star$ using distance measurements, and update $i=i+1$ when the robot's distance to $x_{i,q}^\star$ is within a user-specified tolerance. 
% In the following sections, we demonstrate the performance of the proposed LCA and baselines in realistic Gazebo simulations, and show results on a real robot in our video. We also include numerical simulations in dynamic environments in the video.

% After the robot has moved, we update $t=t+1$ and measure the pose to get $x_{meas}(t)$. We update $i=i+1$ after every $t+T_s$ seconds only if there were no delays in the system. Instead of measuring delays directly, during the online execution, we quantify the robot's progress to $x_p^\star(i)$ using distance measurements, and update $i=i+1$ when the robot's current measured distance to $x_{i, q}^\star$ falls within a user-specified tolerance. Our proposed online execution scheme takes less than $0.01$ seconds to solve on average and can run up to a $100$ Hz. In the following sections, we demonstrate the performance of our proposed LCA and baselines on Gazebo simulations, and show the performance on a real robot in our video. We also include numerical simulations with dynamic environments in our video.

% When commanding the robot online, we use trajectory index $p$ to decide which trajectory the robot should follow and discrete time index $i$ to regulate which state the robot should track, using the closed-loop feedback controller $\mu_p^\star(\cdot)$ for the selected nominal trajectory $p$. Following the same notation convention as in~\autoref{sec:admm-cbf-lca}, we denote the state that the robot selects through heuristic policies to be $x_p^\star(i)$.

 % Then, given the updated $i$, we use a nearest neighbor (NN) search given by

% leading to the smallest deviation between the predicted robot state $x_\text{pred}=f_d(x_\text{meas}, u_\text{cbf})$ and the next nominal state candidates $x^*_{i,p}$ is selected using nearest neighbor search. The updated $p$ and $i$ values are used to compute the new nominal controller. \yifan{Needs edits} 

% we choose a nominal input by doing a nearest neighbor search over predicted next states where ties are broken by choosing the state closer to the center line connecting the initial location to the goal. The nominal input is further modified using a control barrier function and applied to the robot at time step $t$. Using the deviation predicted state and measured state, we determine whether the next nominal input or the same one to account for motor delays and uncertainties. For our online execution, we first select 

% \subsection{Second Order Dubin-CBF}
% A weakness of this method is that it only modulates the linear acceleration in the CBF constraints. Hence, unless the robot is fully maneuverable using angular velocity $\omega$ and considering the angular acceleration, the robot is restricted to avoiding obstacles by increasing or decreasing its linear speed. This restriction leads the robot frequently, and almost certainly, to infeasible conditions, where CBF-QP solvers fail to produce a solution when avoiding dynamic obstacles. However, as in \cite{diffCBF}, solutions for differential drive robots like Fetch, which can only be operated smoothly when accelerations are taken into consideration, are readily available by presenting the kinematics of the robot in the shifted coordinate system, where $a$ is the point of interest on the axis of symmetry of the wheel shaft, 
% \begin{equation}
% \begin{bmatrix}
%  \Dot{x}_1 \\
%  \Dot{x}_2 \\
%  \Dot{v}\\
%  \Dot{\theta}\\
%  \Dot{\omega}
% \end{bmatrix} =
% \begin{bmatrix}
%  vcos\theta-a\omega sin\theta\\
%  vsin\theta+a\omega cos\theta\\
%  u_l-a\omega^2\\
%  \omega\\
%  u_{a}
%  \end{bmatrix}.
%  \label{eq:high order dubin shifted}
% \end{equation}
% Using the shifted differential drive model, $v'$ and $v_n'$ at the center of the wheel axis, given the linear and angular speed at the chosen point $v$, $\omega$, can be computed as
% \begin{equation}
%    |v'| = \sqrt{\dot{x}_1^2+\dot{x}_2^2}=\sqrt{v^2+a^2\omega^2}\\
% \end{equation}
% \begin{equation}
%    v_n' = \nabla_x h(x,t)[ v\cos\theta-a\omega \sin\theta \;\; v\sin\theta+a\omega \cos\theta]^T\\
% \end{equation}
% The modified CBF is now of relative degree 1 to linear/angular acceleration inputs $u_l$ and $u_a$, due to its dependence on $\omega$,
% \begin{equation}
%    p_s' = h(x,t) - \frac{|v'v_n'|}{2a_{max}}\\
% \end{equation}
% \begin{equation}
%    p_r' = h(x,t) + \frac{|v'|}{2a_{max}}v_n'-M(v_{max},a_{max})\\
% \end{equation}


% \section{Integration of LCA with CBF}
% The performance for obstacle avoidance applications using CBF-QP is limited by the quality of its nominal controllers, in cases of complex high order robots, feasible trajectories cannot be produced in real-time. Therefore, approximations have to be made. For example, one approximated nominal control commonly used by first order unicycle model using CBF-QP is the approximated linear dynamics.

% \begin{equation}
% \begin{aligned}
% v_\text{nom} = ||u_\text{nom}^l||_2 \quad \omega_\text{nom} = \frac{\phi}{\Delta t}
% \end{aligned}\label{eq:dubin nominal system}
% \end{equation}

%  Those approximated trajectories are neither smooth nor feasible, causing reasonable robot motions such as swaying and degrading task efficiencies. Some other methods, such as MPC-CBF, choose to tackle the issue of nominal control infeasibility by combining global trajectory design with safety constraints from CBFs. However, the resulted optimization problem become non-convex, which limits the horizon 
%  In this paper, we robustify obstacle avoidance performance of 1st and 2nd order differential drive systems by combining LCA with CBF. LCA serves as the global controller and generates dynamics-feasible trajectories at low frequency without consideration of environmental obstacles. Then CBF, standard or dubin, modifies the trajectory minimally to ensure the safety of the trajectories at real time. 

% We here plan to test and compare the following combinations of LCA with CBF. 

% % \subsection{Standard CBF with 1st Order 2-LCA}
% This algorithm is proposed to achieve collision-free path planning using 1st order differential drive system in Eq.\eqref{eq:low order dubin}. The layered structure of the algorithm is depicted in Figure \ref{fig:2-LCA CBF 1st}, where CBF takes in the trajectory generated by 2-LCA as the nominal control and output modified safe command $[v, \omega]$. When using 1st order dubin CBF, $u_{nom} = [v, \omega]^T$ from 2-LCA can be plugged into Eq \eqref{eq:dubin barrier} directly. However, when using standard CBF, $u_{nom}$ must be converted into velocities in $x_1, x_2$ directions as shown in the following.
% \begin{equation}
%     \begin{aligned}
%         u_{nom}^s = [\dot{x_1},\dot{x_2}]^T = [vcos\theta, vsin\theta]^T
%     \end{aligned}
% \end{equation}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/2-layer velocity admm.png}
%     \caption{2-layer LCA-CBF algorithm for 1st order differential drive system.}
%     \label{fig:2-LCA CBF 1st}
% \end{figure}

% \subsection{Dubin CBF with 2nd Order 2-LCA}
% This algorithm is proposed to achieve collision-free path planning using 2nd order differential drive system in Eq.\eqref{eq:high order dubin}. The layered structure of the algorithm is depicted in Figure \ref{fig:2-LCA CBF 2nd}, where Dubin-CBF, as described in Eq.\eqref{eq:dubin barrier} and \eqref{eq:high order dubin shifted}, takes in the trajectory generated by 2-LCA as the nominal control and output modified safe command $[u_l, u_a]$. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/2-layer acceleration admm.png}
%     \caption{2-layer LCA-CBF algorithm for 2nd order differential drive system.}
%     \label{fig:2-LCA CBF 2nd}
% \end{figure}

% \subsection{Dubin CBF with 2nd Order 3-LCA}
% This algorithm is proposed to achieve collision-free path planning using 2nd order differential drive system in Eq.\eqref{eq:high order dubin}. Unlike the 2-layer variant, 3-LCA CBF, though taken into consideration of robot acceleration limits in acceleration dynamics planning layer implicitly, feeds $u_{nom} = [v, \omega]^T$, explicitly satisfying velocity constraints and implictly satisfying acceleration constraints, into standard or 1st order dubin CBF. The layered structure of the algorithm is depicted in Figure. \ref{fig:3-LCA CBF}. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/3-layer admm.png}
%     \caption{3-layer LCA-CBF algorithm for 2nd order differential drive system.}
%     \label{fig:3-LCA CBF}
% \end{figure}

==> tex/5a-Simulations.tex <==
\section{Numerical Simulations} \label{sec:simulationss}
In this section, we evaluate our proposed methods and compare against $3$ baselines. Each of our baselines represent categories of prior work that consider the problem of robot navigation in a dynamic environment. Our first baseline is MPC-CBF~\cite{mpcdc2021safety} that jointly solves OCPs with a discrete-time CBF constraint and control objectives. We aim to show here that solving without using a layered solution such as is the case of MPC-CBF results in poor performance in practice due to real-time computational constraints. Our second baseline is a custom implementation of MPC with a CBF-QP safety filter. This approach is in the spirit of several prior works~\cite{rosolia2020multi, grandia2021multi, rosolia2022unified, matni2024towards} that use a multirate control architecture solving for a single trajectory at low frequencies while designing tracking controllers that run at higher frequencies. We aim to show that our proposed method is complementary to such approaches and emphasize the benefit to having layered solutions for better performance in practice. Our third and final baseline is CBF-QP~\cite{ames2019control} which is a reactive policy to motivate the need for the careful design of nominal controllers.

In all of the following, we use the $\rho$-update rule described in~\cite[\S3.4.1, equation (3.13)]{boyd2011distributed} to improve convergence of the ADMM algorithm. We provide custom implementations of our ADMM-CBF-LCA and baselines using \texttt{cvxpy}~\cite{diamond2016cvxpy}, CasADI~\cite{} and JAX optimizers~\cite{jax2018github}.  Empirically, we found $\delta=0.8 m$ to be a reasonable interval sizes for Fetch robot navigation tasks.

\subsection{Robot Dynamics}
In this work, we validate our proposed structure and compare it to the listed baselines using differential drive robots. The most commonly used model for differential drive robots like Fetch is the unicycle nonlinear dynamical systems below. 
\begin{equation}
\label{eq:standard unicycle}
    \dot{\xi}=\begin{bmatrix}
        \dot{x}\\\dot{y}\\\dot{\theta}
    \end{bmatrix}=
    \begin{bmatrix}
        \cos{\theta} & 0\\ \sin{\theta} & 0\\ 0 & 1
    \end{bmatrix}
    \begin{bmatrix}
        v \\ \omega
    \end{bmatrix}
\end{equation}

While CBF-QP is easily generalizable in any control affine systems, it suffers from one critical restriction: the CBF has to be of relative degree 1. In other words, the CBF's first time-derivative has to depend on the control input. Since the control input $\omega$ in the standard unicycle model is of relative degree 2 to the CBFs $h_\text{conv}$, HO-CBF-QP using $p(\xi,t)$ of relative degree 1 to control inputs, instead of signed distance function $h(x,y,t)$, is used to construct our CBF filter. The CBFs $p(\xi,t)$ used by 3-dimensional HO-MCBF-QP and HO-CBF-QP in our validations are constructed as the following. 
\begin{equation}
    p(\xi, t) = h(x,y,t) + a\frac{\partial h(x,y,t)}{\partial x}\cos{\theta}+a\frac{\partial h(x,y,t)}{\partial y}\sin{\theta}
    \label{eq:ho barrier function}
\end{equation}

\subsection{Results}

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c}
    \hline
        Algorithms & CR & SR & T & t \\
        \hline
        \textit{ADMM-MCBF-LCA} &  &  &  \\
        \hline
        \textit{MPC-CBF} & $10\%$ & $96.67\%$ & $9.2 \pm 3.8$ & $0.016 \pm 0.02$ \\ 
        \hline
        \textit{MPC-CBF-LCA} &  &  & \\ 
        \hline
        \textit{MCBF-QP} &  &  & \\ 
        \hline
    \end{tabular}
    \caption{\textmd{Comparison of our approach against baselines for $10$ randomly sampled initial conditions per each type of $3$ obstacle scenarios summing to a total of $30$ examples. The first two columns plot the collision rate (CR) and success rates (SR), respectively. The third column $T$ denotes the total time taken to complete tasks on average and $t$ is the execution time for each iteration.}}
    \label{tab:cp}
\end{table}

\subsection{Discussion}

==> tex/5b-Experiments.tex <==
\section{Experiments}\label{sec:experiments}
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
         \includegraphics[width = \textwidth]{img/env_approximation.pdf}
    \vspace{-15pt}
    \caption{\label{fig:env approx}}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
         \includegraphics[width=\textwidth]{img/hospital_trajectories.pdf}
         \vspace{-15pt}
     \caption{\label{fig:hospital-traj}}
    \end{subfigure}
    \vspace{-15pt}
    \caption{\label{fig:online-execution}In~\ref{fig:env approx}, we show boundaries of the obstacle inside hospital Gazebo simulations that are learned using GPDF~\cite{choi2024towards}, and the ellipse approximations used by MPC-CBF solver. In~\ref{fig:hospital-traj}, we plot the results from Gazebo simulations of our approach and $4$ baselines for the indoor environment with unknown obstacles. We observe that ours shown in blue is the only approach that reaches the goal while ensuring safety.}   
    % \vspace{-10pt}
\end{figure}

% \begin{table*}
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%     \hline
%         Horizon ($T$) & Sampling Time ($T_s$) & Avg. Time (secs) \\
%          \hline
%         16 & 0.5 &  \\
%         \hline
%         40 & 0.2 &  \\ 
%         \hline
%         80 & 0.1 &  \\ 
%         \hline
%         160 & 0.05 & \\
%         \hline
%         400 & 0.02 & \\
%         \hline
%     \end{tabular}
%     \caption{We report the time taken to compute $5$ paths for different values of horizon $T$ and $T_s$ on the unicycle model for $100$ randomly sampled initial and goal conditions. In our GitHub repository, we also provide several other dynamics models to test on. \rev{Will make this into a graph for different $T_s$.}
%     }
%     \label{tab:admm}
% \end{table*}
\begin{table}
    \centering
    \begin{tabular}{c|c|c}
    \hline
        Horizon ($T$) & Sampling Time ($T_s$) & Avg. Time (secs) \\
         \hline
        16 & 0.5 &  2.090\\
        \hline
        40 & 0.2 & 7.545 \\ 
        \hline
        80 & 0.1 &  23.175\\ 
        \hline
        160 & 0.05 & 47.635\\
        \hline
        400 & 0.02 & 209.595\\
        \hline
    \end{tabular}
    \caption{We report the time taken to compute $5$ paths for different values of horizon $T$ and $T_s$ on the unicycle model for $5$ randomly sampled initial conditions given the same goal condition. In our GitHub repository, we also provide several other dynamics models to test on.}
    \vspace{-10pt}
    \label{tab:admm}
\end{table}

\begin{table*}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
        Algorithms & QP-solver fail \# $\downarrow$ & Safety \% $\uparrow$ & Task success \% $\uparrow$ & Lin. speed ($\Bar{v}$) $\uparrow$ & Ang. speed ($\Bar{\omega}$) $\downarrow$ & $v$ err. ($e_v$) $\downarrow$ & $\omega$ err. ($e_\omega$) $\downarrow$ \\
         \hline
        \textit{ADMM-MCBF-LCA} & \textbf{0} &  \textbf{100}&  \textbf{100} & \textbf{0.487} & 0.584 & 0.012 & 0.027 \\
        \hline
        \textit{MPC-CBF}  & - & 100 & 0 & 0.100 & 1.303 & 0.011 & 0.074\\ 
        \hline
        \textit{MPC-CBF-LCA} & 0 & 100 & 0 & 0.048 & 0.537 & 0.005 & 0.024 \\ 
        \hline
        \textit{MPC-MCBF-LCA}  & 33 & 100 & 0 & 0.024 & 1.246 & 0.008 & 0.037 \\
        \hline
        \textit{MCBF-QP} & 19 & 60 & 0 & 0.380 & 0.989 & 0.015 & 0.051 \\ 
        \hline
        \textit{MPPI}  & - & 100 & 0 & 0.036 & 0.312 & 0.037 & 0.035\\ 
        \hline
    \end{tabular}
    \caption{\textmd{We report the metrics for all algorithms evaluated from 5 gazebo trials showing in bold the metrics for which our proposed ADMM-MCBF-LCA performed the best. We use $\uparrow$ and $\downarrow$ to indicate if higher or lower is better, respectively. $\Bar{v}$ and $\Bar{\omega}$ are the average linear and angular speeds and their average tracking errors are denoted by $e_{\Bar{v}}, e_{\Bar{\omega}}$. The first three columns indicate algorithm performance in terms of QP solver failure across trials, \% collision-free trials, and \% task completion rate. 
    % Performance of the proposed ADMM-MCBF-LCA with the 4 baselines evaluated from 5 gazebo trials with respect to the robot's mean linear speed $\Bar{v}$, mean angular speed $\Bar{\omega}$, error in tracking linear velocity $e_v$ command, error in tracking angular velocity $e_\omega$ command, total number of solver infeasibility encountered, the collision-free trajectory percentage and the percentage for the robot to reach the goal. All methods compared are updated at 20 Hz frequency, except MPC-CBF, which updates at 5Hz frequency due to runtime limitations. ``failed to solve" means MPC-CBF"converged to a point of local infeasibility".
    }}
    \label{tab:uni}
    \vspace{-20pt}
\end{table*}
\vspace{-1pt}

In this section, we evaluate our proposed method on the differential drive robot Fetch through realistic Gazebo simulations and qualitative hardware experiments. We compare our proposed ADMM-MCBF-LCA against four baselines, each representing a category of prior work on safe real-time robot navigation in dynamic environments. We use metrics such as input tracking error, solver infeasibility, collision-free rate, and task success. For ADMM, we use the $\rho$-update rule described in~\cite[\S3.4.1, equation (3.13)]{boyd2011distributed} to improve convergence. We provide custom implementations of all algorithms using \texttt{cvxpy}~\cite{diamond2016cvxpy}, CasADi~\cite{Andersson2019} and JAX optimizers~\cite{jax2018github}. Empirically, we found $\delta=0.8 m$ to be a reasonable interval size for Fetch robot navigation tasks for our dynamic environment settings. 
% To validate our proposed ADMM-MCBF-LCA framework against existing safe reactive navigation systems, we demonstrate experiments on realistic Gazebo simulations and hardware. The task for the robot is to navigate an unknown indoor hospital environment as shown in Figure~\ref{fig:hospital-traj} starting within the concave obstacle desk and reach the other end of the room. On hardware as shown in Figure~\ref{fig:experiment}, we qualitatively show our experiment in a cluttered indoor environment with a human walking in the robot's exploration space.

% In this section, we evaluate our proposed method on the differential drive robot Fetch and compare it against $4$ baselines. Each of our baselines represents a category of prior work that considers the problem of safe real-time robot navigation in a dynamic environment. We evaluate our approach and baselines using metrics that measure input tracking error, solver infeasibility, safety as measured by collision rate, and task success.

The first baseline is MPC-CBF~\cite{mpcdc2021safety}, which solves OCPs with a discrete-time CBF constraint. The second and third baselines use MPC with CBF-QP and MCBF-QP safety filters, similar to prior multirate control works~\cite{rosolia2020multi, grandia2021multi, rosolia2022unified, matni2024towards}. We demonstrate that our method complements these approaches, highlighting the advantage of layered solutions for better performance. The final reactive baseline, MCBF-QP~\cite{xue2024nominima}, is a reactive policy with a naive single integrator model as its nominal controller, underscoring the importance of well-designed nominal controllers. We also provide a comparison with a sampling-based variant of MPC, biased Model Predictive Path Integral (MPPI)~\cite{biasedMPPI}.
% For the MCBF-QP baseline, we use a naive single integrator model as the nominal controller.

% Our first baseline is MPC-CBF~\cite{mpcdc2021safety} that jointly solves OCPs with a discrete-time CBF constraint and control objectives. Our second and third baselines are MPC with a CBF-QP and MCBF-QP safety filters respectively. These approaches are in the similar vein of several prior works~\cite{rosolia2020multi, grandia2021multi, rosolia2022unified, matni2024towards} that use a multirate control architecture solving for a single trajectory at low frequencies while designing tracking controllers that run at higher frequencies. We aim to show that our proposed method is complementary to such approaches and emphasize the benefit to having layered solutions for better performance in practice. Our final baseline is MCBF-QP~\cite{xue2024nominima} which is a reactive policy to motivate the need for the careful design of nominal controllers.



% \begin{figure}[t]
%     \centering
%     \subfloat[\label{3a}]{
%         \centering  
%         \includegraphics[width=0.5\columnwidth, height=1.4in]{img/env approximation.pdf}
%         \label{fig:env approx}
%     } 
%     % \hfill
%     \subfloat[\label{3b}]{
%         \centering
%         \includegraphics[width=0.5\columnwidth, height=1.4in]{img/hospital trajectories.pdf}
%         \label{fig:hospital-traj}
%     }
%     \caption{In~\ref{fig:env approx}, we show boundaries of the obstacle inside hospital gazebo simulations that are learned using GPDF, and the ellipse approximations used by MPC-CBF solver, we plot the results from Gazebo simulations of our approach and $4$ baselines for the indoor environment with unknown obstacles. We observe that ours shown in blue is the only approach that leads to convergence to the goal while ensuring safety..}   
% \end{figure}

\subsection{Robot Dynamics and Obstacle Definitions}
For all experiments, we model Fetch using the unicycle nonlinear dynamics given as 
\begin{equation}
\label{eq:standard unicycle}
    \dot{x}=\begin{bmatrix}
        \dot{p_x}\\\dot{p_y}\\\dot{\theta}
    \end{bmatrix}=
    \begin{bmatrix}
        \cos{\theta} & 0\\ \sin{\theta} & 0\\ 0 & 1
    \end{bmatrix}
    \begin{bmatrix}
        v \\ \omega,
    \end{bmatrix}
\end{equation}
where $v, \omega$ are the linear and angular speeds such that $v_{max} = 1$m/s, $\omega_{max} = 2$m/s, $v_{min} = \omega_{min} = 0$. The state of the robot consists of 2-D Euclidean position $p_x, p_y$, and orientation $\theta$. 
 
% we use the closed-form nominal controller
% \begin{equation}
% \label{eq: reactive nom}
% \begin{aligned}
% v_\text{nom} = ||u_\text{nom}^l||_2 \quad \omega_\text{nom} = \frac{\psi}{T_s}
% \end{aligned}
% \end{equation}
% to lead the robot toward the goal location, where $\psi$ is the angle difference between the current robot pose $\theta$ and the desired robot pose estimated using the orientation of $u_\text{nom}^l$, and $\Delta t$ is the update timestep of the nominal controller. Note that this reactive nominal control cannot ensure input feasibility. 

To apply the MCBF-QP and CBF-QP approaches, the CBF must have relative degree 1, i.e., the control input must appear in the first time-derivative of the CBF. Since the control input $\omega$ for~\eqref{eq:standard unicycle} is of relative degree 2 to the CBFs used, instead of a signed distance function we use a higher-order CBF % $h(t, p_x, p_y)$, 
(HO-CBF)~\cite{diffBarrier, diffCBF} 
% $p(\xi,t)$ 
of relative degree $1$ with respect to control inputs $v, \omega$. HO-CBF $h_\text{OH}(x, x_o^j)$, shown in Eq.~\eqref{eq:ho barrier function}, is defined on robot position and orientation, where $h(p_x, p_y, x_o^j)$ is the robot's orthonormal distance to the obstacle surface, and $w$ is a scalar weight.
\begin{equation}
\begin{aligned}
 h_\text{OH}(x, x_o^j) = h(p_x,p_y,x_o^j) + w\frac{\partial h(p_x,p_y,x_o^j)}{\partial p_x}\cos{\theta}\\
 +w\frac{\partial h(p_x,p_y,x_o^j)}{\partial p_y}\sin{\theta}
    \label{eq:ho barrier function}   
\end{aligned}
\end{equation}

% to construct our CBF filter. 
% It is noteworthy that HO-CBF, in comparison to signed distance function as CBF, is more difficult to design and tune, and becomes susceptible to the influence of model uncertainty. Many differential drive applications using CBF-QP thus introduce a shifted unicycle model to balance the relative degree differences \cite{diffCBF}\cite{MCBF}. However, the method of shifting the reference point of the robot does not work for all robot dynamics in general. 
Our experiments highlight how judiciously combining a properly designed global nominal controller with a MCBF-QP filter (based on a HO-CBF) can achieve stable and safe navigation in crowded and concave environments. For all methods except MPC-CBF, the obstacle boundaries are obtained using learned Gaussian Process Distance Fields (GPDF)~\cite{choi2024towards}. 
% Obstacle boundaries learned using GPDF cannot be expressed using simple mathematical expressions and thus are impossible to solve as 
Since MPC-CBF requires discrete-time CBF constraints, we instead use ellipse approximations, as shown in~\autoref{fig:env approx}. In our approach, the index $i$ is updated based on progress to $x_{i,p^\star}^\star$ using distance measurements, adjusting for delays within a user-specified tolerance.

% for MPC-CBF.
% For our approach, the index $i$ is incremented every $t+T_s$ seconds, provided there are no system delays. To account for delays, we quantify the robot's progress to $x_{i, q}^\star$ using distance measurements, and update $i=i+1$ when the robot's distance to $x_{i,q}^\star$ is within a user-specified tolerance. 

% The CBFs $p(\xi,t)$ used by 3-dimensional higher order MCBF-QP (HO-MCBF-QP) and HO-CBF-QP in our validations are constructed as the following. 
% \begin{equation}
%     p(\xi, t) = h(x,y,t) + a\frac{\partial h(x,y,t)}{\partial x}\cos{\theta}+a\frac{\partial h(x,y,t)}{\partial y}\sin{\theta}
%     \label{eq:ho barrier function}
% \end{equation}

\subsection{Results}
% We present the results from running our approach and baselines in~\autoref{tab:uni}.
The task for the robot is to navigate an indoor hospital environment as shown in Figure~\ref{fig:hospital-traj} starting within the concave obstacle desk and reach the other end of the room. Among all approaches, only our approach safely navigates the robot to the goal shown in Figure~\ref{fig:hospital-traj}. We summarize metrics in~\autoref{tab:uni}, where $\Bar{v}$, $\Bar{\omega}$, are average linear and angular speeds, $e_{\Bar{v}}, e_{\Bar{\omega}}$ are errors in tracking linear and angular speeds, computed as deviations between commanded and measured inputs. On hardware as shown in Figure~\ref{fig:experiment}, we show our robot safely navigating around a human walking in the robot's exploration space. 
% In Table~\ref{tab:admm}, we report the time taken by our path generation method for different choices of \rev{sampling} times $T_s$ and trajectory horizons $T$.
% $v_t, \omega_t$ are the command input at time $t$ and $v_t^m, \omega_t^m$ are the measured robot states. 
% \begin{equation}
%     \Bar{v}=\frac{1}{T}\sum_{t=0}^T v_t,\  \Bar{\omega}=\frac{1}{T}\sum_{t=0}^T \omega_t, \
%     e_v = \frac{1}{T}\sum_{t=0}^T (v_t-v_t^m)^2 \  e_\omega = \frac{1}{T}\sum_{t=0}^T (\omega_t-\omega_t^m)^2
% \end{equation}

% In the first experiment, we provided Fetch with the task of traveling from an initial location to the goal in a closely-packed gazebo hospital environment with both convex and concave obstacles, simulating daily delivering tasks. In the second experiment, we use real-life experiments using Fetch to compare each method's performance in a dynamic environment with humans walking around. Data collected from the first gazebo simulations are summarized in \autoref{tab:uni}. 
From the results reported, we observe that MCBF-QP controller fails to reach the goal although it is guaranteed to escape local minima. We believe that this is due to large model mismatch from using a naive dynamics model for nominal input design. 
% The high mean angular speed $\Bar{\omega}$ for MCBF-QP compared to ours indicate that reactive methods lead to infeasible inputs. 
Using discrete-time MPC with CBF constraints (MPC-CBF) struggles with navigating Fetch out of concave obstacles due to large tracking errors from low update frequencies. The nonlinear CBF constraints increase runtime, limiting the horizon size; with a horizon of 5, CasADi solvers drop below 5Hz. Additionally, MPC-CBF often fails to find globally optimal solutions, returning infeasible across all trials. As reported in the table~\ref{tab:uni}, MPC-CBF results in large average angular speeds and input tracking errors. Biased MPPI~\cite{biasedMPPI} results in local minima at the concave obstacle region preventing the robot from finding a way out. Among the layered baselines, we find that MPC with CBF-QP outperforms MPC with MCBF-QP resulting in lower input errors and lower average $\Bar{\omega}$. However, neither approaches escape the concave obstacle region to reach the goal. Through the careful design of a nominal feedback law as in~\eqref{eq:nominal-inp}, our proposed ADMM-MCBF-LCA successfully navigates the robot out of the concave obstacle to the goal. In supplementary videos~\footnote{\url{https://www.youtube.com/watch?v=YhL_OHK8AZ8}}, we show real-robot experiments of our approach outperforming all baselines in indoor environments with static and dynamic obstacles.
% As shown in~\autoref{tab:uni}, we report the number of times the QP solver fails during online execution. Since MPC-CBF doesn't use a QP solver but rather a  Layering MPC with CBF-QP resolves the runtime issue but fails in reaching the goal, as MPC without obstacle constraints drives the robot through obstacles. In contrast, ADMM-MCBF-LCA achieves safety and task completion by adapting to feasible trajectories and minimizing tracking errors.

% Among all methods compared, MCBF-QP has mean angular speed $\Bar{\omega}$, and error nearly twice as large as that of the ADMM-MCBF-LCA in angular speed tracking. The use of the infeasible nominal controller in \eqref{eq: reactive nom} results in high angular speed,  makes it difficult to track input commands, and consequently failed in reaching the goal despite MCBF filter eliminating all local minima. Besides, solving a discrete-time MPC to guarantee safety (MPC-CBF) fails in navigating Fetch out of concave obstacles due to high tracking errors caused by the low update frequencies. Discrete-time CBF constraints are nonlinear in general, and scale up the runtime drastically when the horizon increases, thus limiting the available horizon size of MPC-CBF. With a horizon size of 5, CasADI solvers' update frequency fails below 5Hz. Additionally, MPC-CBF solvers have difficulty in finding globally optimal solutions given complicated CBF constraints. CasADI solvers only managed to "Converge to a point of local infeasibility" during all trials. Lastly, MPC forming a layered structure with CBF-QP filters failed in task completion despite resolving the runtime limitation of MOC-CBF. MPC with no obstacle constraints insists on driving the robot back to the shortest trajectory to the goal of penetrating through the front desk. The tangent space modulation conducted by MCBF-QP is thus canceled out. ADMM-MCBF-LCA achieves optimal performance in terms of safety and task completion as it actively adapts to the different globally converged feasible trajectories when MCBF-QP guides the robot outside the front desk, thus minimizing the effects of model uncertainties and tracking errors on the robot while taking full advantage of local-minimum-free MCBF filter. 


% Further, we observe that even in ideal environments, the solver returns infeasible solutions due to real-time computational constraints. 
% and the inherent continuous dynamics of robot motion. 

% MPC-CBF with . MPC-CBF-LCA and MPC-MCBF-LCA with horizon size of 20 and dt of 0.1. LI standards for "Converged to a point of local infeasibility".

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{img/hospital trajectories.pdf}
%     \caption{}
%     \label{fig:enter-label}
% \end{figure}

==> tex/6-Conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
We conclude that addressing the combined challenges of input feasibility, safety, and real-time computation for robot navigation in environments with moving obstacles, requires layered solutions for robustness and task performance. Our proposed ADMM-MBCF-LCA generated a library of feasible paths offline, to construct a nominal feedback law that is easy to track for our MCBF filter to ensure safety.
% and online path selector and safety layer to handle the above-mentioned challenges. 
We demonstrated experiments on realistic Gazebo simulations and hardware showing our approach outperforming baselines in terms of reaching the goal while generating safe and feasible inputs. The baselines representing prior work on reactive methods, and end-to-end solvers perform worse than all layered approaches. We also observed that due to the computation-performance tradeoffs, nonlinear MPC based LCAs do not reach the goal and are stuck in local minima. In future work, we plan to address the question of ADMM convergence rigorously for nonlinear systems. 
